Mixed-Precision Neural Networks: A Survey

Mixed-precision Deep Neural Networks achieve the energy efficiency and throughput needed for hardware deployment, particularly when the resources are limited, without sacrificing accuracy. However, the optimal per-layer bit precision that preserves accuracy is not easily found, especially with the abundance of models, datasets, and quantization techniques that creates an enormous search space. In order to tackle this difficulty, a body of literature has emerged recently, and several frameworks that achieved promising accuracy results have been proposed. In this paper, we start by summarizing the quantization techniques used generally in literature. Then, we present a thorough survey of the mixed-precision frameworks, categorized according to their optimization techniques such as reinforcement learning and quantization techniques like deterministic rounding. Furthermore, the advantages and shortcomings of each framework are discussed, where we present a juxtaposition. We finally give guidelines for future mixed-precision frameworks.

==> Mixed Precision Frameworks Survey/Summary_Fig.tex <==
%\begin{landscape}
\begin{figure}
\centering
\begin{tikzpicture}
\path[mindmap,concept color=black,text=white,level 2 concept/.append style=
      {every child/.style={concept color=blue!70},sibling angle=-42}]
      
    node[concept] {Mixed Precision\\ Frameworks}
    [clockwise from=140]
    
    child[concept color=orange, yshift=-6cm, xshift=2.5cm grow=90,font=\fontsize{10pt}{16pt}]{ 
        node[concept] {Gradient-Based\\Optimization}
            [clockwise from=130]
        % child {node[concept] {\cite{}} }
        child {node[concept] {SLWP(\cite{lacey2018stochastic})} }
        child {node[concept] {DQ (\cite{uhlich2019differentiable})} }
        child {node[concept] {OBACWA (\cite{zhe2019optimizing})} }
        child {node[concept, xshift=5] {Bayesian Bits (\cite{van2020bayesian})}
        }}
    child[concept  color=orange, grow=-90, xshift=2cm] 
    { 
        node[concept] {Heuristic-Based\\Optimization}
            [clockwise from=170]
        % child {node[concept] {\cite{}} }
        child {node[concept] {AQ(\cite{zhou2018adaptive})} }
        child {node[concept] {PDB (\cite{chu2019mixed})} }
        child {node[concept] {HAWQ (\cite{dong2019hawq})}}
        child {node[concept] {HAWQ-V3 (\cite{yao2021hawq})}}
        child {node[concept] {Hybrid-Net (\cite{chakraborty2020constructing})}}  
        child {node[concept] {ZeroQ (\cite{cai2020zeroq})}}
        child {node[concept] {HAWQ-V3 (\cite{yao2021hawq})}}
        child {node[concept] {MPQNNCO (\cite{chen2021towards})}}
        child {node[concept] {OPQ (\cite{hu2021opq})}
        } }
    child[concept  color=orange, grow=0 xshift=3.5cm,yshift=3cm]
    { 
        node[concept] {Meta-Heuristic-Based\\Optimization}
            [clockwise from=63]
        child {node[concept]{DNAS (\cite{wu2018mixed})} }
        child {node[concept]{JASQ (\cite{chen2018joint})} }
        child {node[concept] {MPNASEE (\cite{pan2019})} }
        child {node[concept] {APQ (\cite{wang2020apq})}}
        child {node[concept, xshift=5] {BP-NAS (\cite{yu2020search})}}
        child {node[concept, yshift=-7] {HMQ (\cite{habi2020hmq})}}
        child {node[concept] {EdMIPS (\cite{cai2020rethinking})}}
        child {node[concept, yshift=4] {EvoQ (\cite{evoq})}}
        child {node[concept, xshift=40, grow=20, yshift=7] {Bit-Mixer (\cite{bulat2021bit})}}}
    child[concept  color=orange, grow=130, xshift=3.5cm,yshift=0.5cm]
    { 
        node[concept] {RL-Based\\Optimization}
            [clockwise from=60]
        child {node[concept, yshift=-15, xshift=10]{ReLeQ (\cite{elthakeb2018releq})} }
        child {node[concept] {HAQ (\cite{wang2019haq})} }
        child {node[concept] {AutoQ (\cite{lou2019autoq})}}
        child {node[concept] {ADRL (\cite{ning2020simple})}}
};
\end{tikzpicture}
\caption{Mixed Precision Frameworks grouped according to their optimization techniques.}
\label{mxdpdnn}
\end{figure}
%\end{landscape}
 
 

==> Mixed Precision Frameworks Survey/Table_inter.tex <==
\begin{table}[]
\centering
\caption{Summary of Mixed Precision Frameworks, where at least weights are quantized with mixed bit precision. In "XWYA", "XW" and "YA" stand for the (average) \# of bits of weights and activations respectively. "X"/"Y"="F" when "W"/"A" take "Flexible" precision assignments layer-wise. "QOP"=quantization as an optimization problem. "DS"=Differentiable Search. "ES"=Evolutionary Search.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Precision Budget\\ (in bits)\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 97.68 & \multicolumn{2}{c|}{10} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 98.31 & \multicolumn{2}{c|}{20} \\ \cline{7-11} 
 &  &  &  & \multirow{-3}{*}{MNIST} & \multirow{-3}{*}{Similar to LeNet-5} & \multicolumn{2}{c|}{8W8A} & 98.86 & \multicolumn{2}{c|}{40} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 51.46 & \multicolumn{2}{c|}{14} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 52.31 & \multicolumn{2}{c|}{28} \\ \cline{7-11} 
\multirow{-7}{*}{SLWP'18} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Gradient-Based\end{tabular}} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-7}{*}{Mixed} & \multirow{-3}{*}{ImageNet} & \multirow{-3}{*}{AlexNet \footnote{1st layer is kept in full precision}} & \multicolumn{2}{c|}{8W8A} & 52.54 & \multicolumn{2}{c|}{56} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\% \\Accuracy \end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\Savings \footnote{Baseline: Equal bit-width quantized models across all layers}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet \footnote{\label{fc16}Fully connected layers are kept in 16-bit precision} & \multicolumn{2}{c|}{FW32A} & 99.50 & \multicolumn{2}{c|}{x1.84} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.68 & \multicolumn{2}{c|}{x1.68} \\ \cline{6-11} 
 &  &  &  &  & GoogLeNet \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.60 & \multicolumn{2}{c|}{x1.16} \\ \cline{6-11} 
\multirow{-5}{*}{AQ'18} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 \footref{fc16}& \multicolumn{2}{c|}{FW32A} & 99.71 & \multicolumn{2}{c|}{x1.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ (or Computational) \footnote{When activations are quantized along with the weights, the computational savings are reported rather than model size savings}\\ Savings \footnote{\label{size}Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{} & 92.72 & \multicolumn{2}{c|}{x11.6} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-56 & \multicolumn{2}{c|}{} & 94.57 & \multicolumn{2}{c|}{x14.6} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-10} & ResNet-110 & \multicolumn{2}{c|}{\multirow{-3}{*}{FW32A \footnote{\label{res1}Activations, the 1st and the last layer are kept in full precision}}} & 95.07 & \multicolumn{2}{c|}{x12.5} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 71.21 & \multicolumn{2}{c|}{x11.2} \\ \cline{7-11} 
 &  &  &  &  & \multirow{-2}{*}{ResNet-18 \footnote{\label{res3}ReLU-only preactivation}} & \multicolumn{2}{c|}{FWFA \footnote{\label{res2}1st and last layer are kept in full precision}} & 71.01 & \multicolumn{2}{c|}{x33.2} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 74.61 & \multicolumn{2}{c|}{x10.6} \\ \cline{7-11} 
\multirow{-8}{*}{DNAS'18} & \multirow{-8}{*}{DS} & \multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-8}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \multirow{-2}{*}{ResNet-34 \footref{res3}} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 74.21 & \multicolumn{2}{c|}{x40.8} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footnote{\label{accloss}Compared to the full precision model}\end{tabular} & \multicolumn{2}{c|}{Speedup \footnote{On conventional hardware using TVM compiler. Baseline: 8-bit precision models for inference}} \\ \cline{5-11} 
 &  &  &  & \multirow{2}{*}{ImageNet} & AlexNet & \multicolumn{2}{c|}{5W32A} & 0.08 & \multicolumn{2}{c|}{x3.95} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{6.43W32A} & 0.26 & \multicolumn{2}{c|}{x1.24} \\ \cline{5-11} 
 &  &  &  &  & SimpleNet & \multicolumn{2}{c|}{5W32A} & 0.30 & \multicolumn{2}{c|}{x1.92} \\ \cline{6-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{2.81W32A} & 0.12 & \multicolumn{2}{c|}{x3.27} \\ \cline{6-11} 
 &  &  &  &  & VGG-11 & \multicolumn{2}{c|}{6.44W32A} & 0.17 & \multicolumn{2}{c|}{x1.53} \\ \cline{6-11} 
 &  &  &  & \multirow{-4}{*}{CIFAR-10} & VGG-16 & \multicolumn{2}{c|}{7.25W32A} & 0.10 & \multicolumn{2}{c|}{-} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet-5 & \multicolumn{2}{c|}{2.25W32A} & 0.00 & \multicolumn{2}{c|}{x2.76} \\ \cline{5-11} 
\multirow{-9}{*}{ReLeQ'18} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}LSTM-based\\ RL\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{None} & SVHN & SVHN-10 & \multicolumn{2}{c|}{4.8W32A} & 100 & \multicolumn{2}{c|}{x2.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{The weights of the output layer are left in full precision in experiments on CIFAR-10\/100 and Pascal VOC, and the weights of the input and output layers are left in full precision in the experiments on ImageNet}\end{tabular}} & \multicolumn{3}{c|}{Top-1\% Accuracy} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{W4A} & \multicolumn{3}{c|}{90.54} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-10} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{93.22} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{3.82W4A} & \multicolumn{3}{c|}{64.28} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-100} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{71.53} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{1.10W2A} & \multicolumn{3}{c|}{53.18} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{1.42W2A} & \multicolumn{3}{c|}{65.03} \\ \cline{5-11} 
 &  &  &  &  & SSD-300 & \multicolumn{2}{c|}{1.22W2A} & \multicolumn{3}{c|}{62.21} \\ \cline{6-11} 
\multirow{-9}{*}{PDB'19} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based on\\ input separability\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{Fixed} & \multirow{-2}{*}{Pascal VOC} & Faster R-CNN & \multicolumn{2}{c|}{1.52W4A} & \multicolumn{3}{c|}{74.52} \\ \hline
{\color[HTML]{000000} } &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
{\color[HTML]{000000} } &  &  &  & CIFAR-10 \footnote{\label{memconst}Without constraints, and the networks are initialized with a pre-trained floating point network} & ResNet-20 \footnote{\label{uniform}With best parametrization of uniform DQ} & \multicolumn{2}{c|}{} & 92.60 & \multicolumn{2}{c|}{-} \\ \cline{5-6} \cline{9-11} 
{\color[HTML]{000000} } &  &  &  &  & MobileNet-V2 \footref{uniform} & \multicolumn{2}{c|}{} & 70.59 & \multicolumn{2}{c|}{x4.21} \\ \cline{6-6} \cline{9-11} 
\multirow{-4}{*}{{\color[HTML]{000000} DQ'19}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Gradient-Based\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & \multirow{-2}{*}{ImageNet \footref{memconst}} & ResNet-18 \footref{uniform} & \multicolumn{2}{c|}{\multirow{-3}{*}{FWFW}} & 70.66 & \multicolumn{2}{c|}{x4.24} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Constraint\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Savings \footnote{Baseline: 8W8A models with energy and latency constraints, 32W32A models with model size constraint}\end{tabular} \\ \cline{5-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{edge}Edge Accelerator} & \multicolumn{2}{c|}{6.8W5.42A} & 70.58 &  & x1.66 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{cloud}Cloud Accelerator} & \multicolumn{2}{c|}{5.73W4.77A} & 69.97 &  & x1.95 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{bitfusion}BitFusion} & \multicolumn{2}{c|}{FWFA} & 70.40 &  & x1.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{edge} & \multicolumn{2}{c|}{5.86W6.10A} & 71.89 &  & x1.4 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{cloud} & \multicolumn{2}{c|}{4.92W5.29A} & 71.85 & \multirow{-5}{*}{Latency} & x1.45 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 \footref{bitfusion} & \multicolumn{2}{c|}{FWFA} & 70.37 & Energy & x1.9 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FWFA} & 71.74 &  & x7.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{3.85WFA} & 71.47 &  & x7.47 \\ \cline{6-9} \cline{11-11} 
\multirow{-10}{*}{HAQ'19} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}RL w/\\ budget constraints\end{tabular}} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\\ Vector Quant.\end{tabular}} & \multirow{-10}{*}{Mixed} & \multirow{-9}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 76.14 & \multirow{-3}{*}{Model Size} & x8.03 \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{w-s}In terms of weight compression. Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{4.05W4A \footnote{fixed 4 bits are used for activations in all layers except the 1st and last, where 8 bits are used}} & 92.22 & \multicolumn{2}{c|}{x13.11} \\ \cline{5-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{3.43W4.11A} & 75.52 & \multicolumn{2}{c|}{x12.04} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.48 & \multicolumn{2}{c|}{x12.28} \\ \cline{6-11} 
\multirow{-5}{*}{HAWQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hessian\\ Spectrum\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Fixed/Mixed} & \multirow{-3}{*}{ImageNet} & SqueezeNet & \multicolumn{2}{c|}{FWFA} & 68.02 & \multicolumn{2}{c|}{x9.25} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{\label{kernel}Kernel-wise quantization results are reported}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy \footnote{Resource-constrained experiments}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footnote{Baseline: 16W16F models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{3.32W4.12A} & 69.78 & \multicolumn{2}{c|}{x4.06} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4.02W3.93A} & 74.47 & \multicolumn{2}{c|}{x3.86} \\ \cline{6-11} 
 &  &  &  &  & SqueezeNet-V1 & \multicolumn{2}{c|}{3.76W4.05A} & 56.49 & \multicolumn{2}{c|}{x3.06} \\ \cline{6-11} 
\multirow{-5}{*}{AutoQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hierarchical\\ deep RL\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{3.67W4.14A} & 70.79 & \multicolumn{2}{c|}{x3.43} \\  \hline
 \end{tabular}%
}
%\afterpage{\clearpage}
\end{table}


\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\
\hline
  &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ Savings \footnote{\label{mbnet}Baseline: 8-bit precision quantized MobileNet-V2}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footref{mbnet}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-100 & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 68.38 & x3.26 & x3.49 \\ \cline{5-11} 
\multirow{-3}{*}{MPNASEE'19} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ \\ energy constraints\\ and a proxy task\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 77.84 & x5.09 & x5.19 \\ \hline
&  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Giga Bit\\ Operation \\ Count Savings \footnote{Of full precision model}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet-5 \footnote{\label{logit}Output logits left in full precision}& \multicolumn{2}{c|}{FWFA} & 99.30 & \multicolumn{2}{c|}{x277.78} \\ \cline{5-11} 
 &  &  &  & CIFAR-10  & VGG-7 \footref{logit}& \multicolumn{2}{c|}{FWFA} & 93.23 & \multicolumn{2}{c|}{x196.08} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 \footref{logit}& \multicolumn{2}{c|}{FWFA} & 69.36 & \multicolumn{2}{c|}{x51.81} \\ \cline{6-11} 
\multirow{-5}{*}{Bayesian Bits'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Variational\\ inference\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & MobileNet-V2 \footref{logit}& \multicolumn{2}{c|}{FWFA} & 72 & \multicolumn{2}{c|}{x16} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top 1-\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Bit Operations\\ Savings \footnote{Baseline: 4W4A models}\end{tabular}} \\ \cline{5-11} 
\multirow{-3}{*}{APQ'20} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Predictor-based\\ES w/ budget\\ constraints\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Their model & \multicolumn{2}{c|}{FWFA} & 75.1 & \multicolumn{2}{c|}{x1.23} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy (or mAP) \footnote{mAP is used for COCO dataset}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bit Operations\\ Budget\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{4W3.9A} & 92.30 & 4 & x10.19 \\ \cline{5-11} 
 &  &  &  & ImageNet & ResNet-50 & \multicolumn{2}{c|}{-} & 76.67 & 4 & - \\ \cline{5-11} 
\multirow{-4}{*}{BP-NAS'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ complexity\\ constraints\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining \\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & Microsoft COCO & \begin{tabular}[c]{@{}c@{}}ResNet-50 \\ (faster R-CNN)\end{tabular} & \multicolumn{2}{c|}{3.84W4.31A} & 0.358 & 4 & - \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\%Degradation\\ Memory\\ Compression \footnote{Baseline: XNOR network}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footnote{\label{identity}With identity shortcut connections at each layer} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.88 & \multicolumn{2}{c|}{47} \\ \cline{6-11} 
 &  &  &  &  & ResNet-32 \footref{identity} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 64.45 & \multicolumn{2}{c|}{31} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-100} & VGG-15 & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.38 & \multicolumn{2}{c|}{50} \\ \cline{5-11} 
\multirow{-5}{*}{Hybrid-Net'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based\\ on PCA\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & ImageNet & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 62.73 & \multicolumn{2}{c|}{20} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 92.43 & \multicolumn{2}{c|}{x11.06} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.45 & \multicolumn{2}{c|}{x13.1} \\ \cline{6-11} 
 &  &  &  &  & EfficientNet-B0 & \multicolumn{2}{c|}{FW8A} & 74.6 & \multicolumn{2}{c|}{x11.97} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FW8A} & 69.88 & \multicolumn{2}{c|}{x10.68} \\ \cline{6-11} 
\multirow{-6}{*}{HMQ'20} & \multirow{-6}{*}{DS} & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-6}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{FWFA} & 70.9 & \multicolumn{2}{c|}{x8.05} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{Using efficient composite convolution with respect to vanilla parallel convolutions}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{AlexNet} & \multicolumn{2}{c|}{2W2A} & 59.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{-}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 68 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & 67 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-18} & \multicolumn{2}{c|}{2W2A} & 65.9 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{GoogLeNet} & \multicolumn{2}{c|}{2W2A} & 67.8 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.45}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-50} & \multicolumn{2}{c|}{2W2A} & 72.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
\multirow{-16}{*}{EdMIPS'20} & \multirow{-16}{*}{DS} & \multirow{-16}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-16}{*}{Mixed} & \multirow{-15}{*}{ImageNet} & \multirow{-3}{*}{Inception-V3} & \multicolumn{2}{c|}{2W2A} & 72.4 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{size}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{} & 77.43 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{} & 72.85 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ShuffleNet & \multicolumn{2}{c|}{} & 62.90 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-152 & \multicolumn{2}{c|}{} & 77.88 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{} & 78.76 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & SqueezeNext & \multicolumn{2}{c|}{} & 68.17 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-7}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{} & 71.30 & \multicolumn{2}{c|}{x5.34} \\ \cline{5-6} \cline{9-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{} & 93.87 & \multicolumn{2}{c|}{x5.20} \\ \cline{5-6} \cline{9-11} 
\multirow{-10}{*}{ZeroQ'20} & \multirow{-10}{*}{Pareto Frontier} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-10}{*}{Fixed} & Microsoft COCO & RetinaNet & \multicolumn{2}{c|}{\multirow{-9}{*}{FW6A}} & 35.9 & \multicolumn{2}{c|}{x6.00} \\ \hline
 

 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footref{accloss}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{bl}Baseline: 32W32F}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.30} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.10} \\ \cline{6-11} 
\multirow{-4}{*}{ADRL'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Deep RL w/\\ compression\\ ratio constraint\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{None} & \multirow{-2}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.00} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \multicolumn{3}{c|}{Top-1\% Accuracy \footnote{Random per layer bit selection}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{65.8} \\ \cline{6-11} 
 &  &  &  &  & ResNet-34 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{70.5} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{73.2} \\ \cline{6-11} 
\multirow{-5}{*}{Bit-Mixer'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}3-stage\\ optimization on\\ Meta-Network\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \begin{tabular}[c]{@{}c@{}}EBN \\ 4:4:4:4\end{tabular} & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{72.1} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{2.99W32A} & 57.09 & \multicolumn{2}{c|}{x138.96} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 & \multicolumn{2}{c|}{2.92W32A} & 71.39 & \multicolumn{2}{c|}{x195.87} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{3.26W32A} & 70.83 & \multicolumn{2}{c|}{x23.26} \\ \cline{6-11} 
\multirow{-5}{*}{OPQ'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Codebook\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{3.25W32A} & 76.41 & \multicolumn{2}{c|}{x38.03} \\ \hline

\end{tabular}
}
\end{table}

==> Mixed Precision Frameworks Survey/Table_new.tex <==


\begin{table}[hbt!]
\caption{Some results of RL-based and gradient-based (underlined) mixed precision frameworks, where at least weights have mixed precision.}
\label{tab:my-table11}
\resizebox{\textwidth}{!}
{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Framework & \begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular} & \begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular} & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Top 1\%\\ Accuracy\end{tabular} & Savings \\ \hline
\multirow{3}{*}{ReLeQ*} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{3}{*}{None} & ImageNet & AlexNet & 63.22 & 3.95x (speedup) \tablefootnote{\label{fn1}On conventional hardware using TVM compiler. Baseline: 8-bit precision models for inference} \\ \cline{4-7} 
 &  &  & Cifar-10 & VGG-16 & 93.46 & - \\ \cline{4-7} 
 &  &  & MNIST & LeNet & 99.4 & 2.76x (speedup) \footref{fn1}\\ \hline
\multirow{3}{*}{HAQ} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{3}{*}{Mixed} & \multirow{3}{*}{ImageNet} & ResNet-50 & 76.14 \tablefootnote{With model size constraints} & 8.03x (Model Size) \tablefootnote{\label{fn2}Baseline: 8W8A models with energy and latency constraints, 32W32A models with model size constraint} \\ \cline{5-7} 
 &  &  &  & MobileNet-V1 \tablefootnote{BitFusion} & 70.90 \tablefootnote{With energy constraints} & 1.16x (Energy) \footref{fn2} \\ \cline{5-7} 
 &  &  &  & MobileNet-V2 \tablefootnote{BISMO Edge accelerator} & 71.89 \tablefootnote{With latency constraints} & 1.4x (Latency) \footref{fn2} \\ \hline
AutoQ & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \end{tabular} & Mixed & ImageNet & ResNet-50 & 74.47 \tablefootnote{With resource-constraints} & 3.86x (Latency) \tablefootnote{Baseline: 16W16F models} \\ \hline
ADRL* & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \end{tabular} & {None} & ImageNet & ResNet-50 & 83.2 & 10x (Model Size) \tablefootnote{\label{bl}Baseline: 32W32F} \\ \hline
\multirow{2}{*}{\underline{SLWP}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & AlexNet \tablefootnote{1st layer is kept in full precision} & 52.54 \tablefootnote{Precision budget: 56} & - \\ \cline{4-7} 
 &  &  & MNIST & Similar to LeNet-5 & 98.86 \tablefootnote{Precision budget: 40} & - \\ \hline
\multirow{2}{*}{\underline{DQ}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet \tablefootnote{\label{memconst}Without constraints, and the networks are initialized with a pre-trained floating point network} & ResNet-18 \tablefootnote{\label{uniform}With best parametrization of uniform DQ} & 70.66 & 4.24x (Model Size)\tablefootnote{In terms of weight compression. Baseline: 32W32A models\label{w-s}}\\ \cline{4-7} 
 &  &  & Cifar-10 \footref{memconst} & ResNet-20 \footref{uniform} & 92.60 & - \\ \hline
\underline{OBACWA} & \begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular} & Mixed & ImageNet & ResNet-50 & 74.8 & 4x (Model Size) \footref{bl} \\ \hline
\multirow{3}{*}{\underline{Bayesian Bits}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{3}{*}{Mixed} & ImageNet & MobileNet-V2 & 72.00 \tablefootnote{\label{logit}Output logits left in full precision} & 16x (GbOp) \footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & VGG-7 & 93.23 \footref{logit} & 196.08x (GbOp) \footref{bl} \\ \cline{4-7} 
 &  &  & MNIST & LeNet-5 & 99.30 \footref{logit} & 277.78x (GbOp)\footref{bl} \\ \hline
 \end{tabular}
}
\end{table}



\begin{table}[hbt!]
\caption{Some results of heuristic-based mixed precision frameworks, where at least weights have mixed precision.}
\label{tab:my-table12}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Framework & \begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular} & \begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular} & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Top 1\%\\ Accuracy\end{tabular} & Savings \\ \hline
AQ & \begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular} & None & ImageNet & ResNet-50 \tablefootnote{Fully connected layers are kept in 16-bit precision} & 99.71 & 1.18x (Model Size)\tablefootnote{Baseline: Equal bit-width quantized model across all layers} \\ \hline
\multirow{3}{*}{PDB} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\end{tabular}} & \multirow{3}{*}{Fixed} & ImageNet & ResNet-18 \tablefootnote{The weights of
the input and output layers are left in full precision} & 65.03 & - \\ \cline{4-7} 
 &  &  & Cifar-10 & VGG-7 \tablefootnote{\label{pdb}The weights of the output layer are left in full precision} & 93.22 \tablefootnote{\label{manual}With manual fine-tuning} & - \\ \cline{4-7} 
 &  &  & Cifar-100 & VGG-7 \footref{pdb} & 71.53 \footref{manual} & - \\ \hline
HAWQ-V2 & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & Inception-V3 & 75.98 & 12.04x (Model Size)\footref{w-s} \\ \hline
\multirow{3}{*}{HAWQ-V3} &\multirow{3}{*}{ \begin{tabular}[c]{@{}c@{}}Retraining/\\Post-training\\ Deterministic\end{tabular}} & \multirow{3}{*}{Fixed/Mixed} & \multirow{3}{*}{ImageNet} & \multirow{3}{*}{ResNet-50} \tablefootnote{All results reported with distillation} & 77.58 & 1.15x (Model Size)\tablefootnote{Baseline: INT8 for weights and activations, with high model size constraint} \\ 
\cline{6-7} 
 &  &  &  &  & 76.97 & 1.13x (Speed)\tablefootnote{Baseline: INT8 for weights and activations, with high latency constraint} \\ 
\cline{6-7} 
 &  &  &  &  & 76.76 & 1.25x (BOPS)\tablefootnote{Baseline: INT8 for weights and activations, with high BOPS constraint} \\
\hline
\multirow{2}{*}{Hybrid-Net*} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic
\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & ResNet-18 & 62.73 & 0.20x (Memory Compression)\tablefootnote{\label{mc1}Baseline: XNOR network}\\ \cline{4-7} 
 &  &  & Cifar-100 & \begin{tabular}[c]{@{}c@{}}ResNet-32 \tablefootnote{\label{identity}With identity shortcut connections at each layer}\\ \tablefootnote{\label{res2}1st and last layer are kept in full precision}\end{tabular} & 64.45 & 0.31x (Memory Compression)\footref{mc1}\\ \hline
\multirow{2}{*}{ZeroQ} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular}} & \multirow{2}{*}{Fixed} & ImageNet & Inception-V3 & 78.76 & 5.34x (Model Size)\footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & ResNet-20 & 93.87 & \begin{tabular}[c]{@{}c@{}}5.20x\\ (Model Size)\\ \footref{bl}\end{tabular} \\ \hline
OPQ & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & None & ImageNet & ResNet-50 & 76.41 & 38.03x (Model Size)\footref{w-s} \\ \hline
MPQNNCO & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & ResNet-50 & 75.28 & 12.24x (Model Size)\footref{w-s} \\ \hline
\end{tabular}%
}
\end{table}



\begin{table}[h!]
\caption{Some results of meta-heuristic-based mixed precision frameworks, where at least weights have mixed precision.}
\label{tab:my-table13}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Framework & \begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular} & \begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular} & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Top 1\%\\ Accuracy\end{tabular} & Savings \\ \hline
\multirow{2}{*}{DNAS} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{2}{*}{None/Mixed} & ImageNet & \begin{tabular}[c]{@{}c@{}}ResNet-34 \tablefootnote{\label{res3}ReLU-only preactivation}\\ \tablefootnote{\label{res1}Activations, the 1st and the last layer are kept in full precision}\end{tabular} & 74.61 & 10.6x (ModelSize)\footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & \begin{tabular}[c]{@{}c@{}}ResNet-110\\ \footref{res1}\end{tabular} & 95.07 & 12.5x (Model Size) \footref{bl} \\ \hline
\multirow{2}{*}{JASQ} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular}} & \multirow{2}{*}{None} & ImageNet & ResNet-152 \footref{res2} & 78.86 & 5.16x(Model Size) \footref{w-s} \\ \cline{4-7} 
 &  &  & Cifar-10 & JASQNet & 97.1 & - \\ \hline
\multirow{2}{*}{MPNASEE} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & Theirs-Base & 71.77 & \begin{tabular}[c]{@{}c@{}}2.67x (Energy)\\ 2.99x (Latency) \tablefootnote{\label{mbnet}Baseline: 8-bit precision quantized MobileNet-V2}\end{tabular} \\ \cline{4-7} 
 &  &  & Cifar-100 & Theirs-Base & 78.73 & \begin{tabular}[c]{@{}c@{}}4.21x (Energy)\\ 4.41x (Latency) \footref{mbnet}\end{tabular} \\ \hline
APQ & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & Their model  & 75.1 & 1.23x (BitOp)\footref{mbnet}\\ \hline
\multirow{2}{*}{BP-NAS} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining \\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & ResNet-50 & 76.67 & 71.65x (BitOp)\footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & ResNet-20 & 92.30 & 10.19x (Model Size)\footref{w-s}\\ \hline
{HMQ} & {\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & {Mixed} & ImageNet & ResNet-50 & 75.73 & 11.1x (Model Size)\footref{w-s} \\ \hline
 %&  &  & Cifar-10 & ResNet-18 & 92.43 & \begin{tabular}[c]{@{}c@{}}11.06x\\ (Model\\Size)\footref{w-s}\end{tabular} \\ \hline
EdMIPS & \begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\end{tabular} & Mixed & ImageNet & Inception-V3 & 72.4 & 3.85x (Model Size)\tablefootnote{Using efficient composite convolution with respect to vanilla parallel convolutions} \\ \hline
EvoQ & \begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular} & Fixed & ImageNet & ResNet-101 & 76.76 & 8x (Model Size) \footref{w-s}\\ \hline
Bit-Mixer & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & ResNet-50 \tablefootnote{Random per layer bit width selection} & 73.2 & - \\ \hline
\end{tabular}%
}
\end{table}

==> Mixed Precision Frameworks Survey/Table_old.tex <==
\begin{table}[]
\centering
\caption{Summary of Mixed Precision Frameworks, where at least weights are quantized with mixed bit precision. In "XWYA", "XW" and "YA" stand for the (average) \# of bits of weights and activations respectively. "X"/"Y"="F" when "W"/"A" take "Flexible" precision assignments layer-wise. "QOP"=quantization as an optimization problem. "DS"=Differentiable Search. "ES"=Evolutionary Search.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Precision Budget\\ (in bits)\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 97.68 & \multicolumn{2}{c|}{10} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 98.31 & \multicolumn{2}{c|}{20} \\ \cline{7-11} 
 &  &  &  & \multirow{-3}{*}{MNIST} & \multirow{-3}{*}{Similar to LeNet-5} & \multicolumn{2}{c|}{8W8A} & 98.86 & \multicolumn{2}{c|}{40} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 51.46 & \multicolumn{2}{c|}{14} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 52.31 & \multicolumn{2}{c|}{28} \\ \cline{7-11} 
\multirow{-7}{*}{SLWP'18} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-7}{*}{Mixed} & \multirow{-3}{*}{ImageNet} & \multirow{-3}{*}{AlexNet \footnote{1st layer is kept in full precision}} & \multicolumn{2}{c|}{8W8A} & 52.54 & \multicolumn{2}{c|}{56} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\% \\Accuracy \end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\Savings \footnote{Baseline: Equal bit-width quantized models across all layers}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet \footnote{\label{fc16}Fully connected layers are kept in 16-bit precision} & \multicolumn{2}{c|}{FW32A} & 99.50 & \multicolumn{2}{c|}{x1.84} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.68 & \multicolumn{2}{c|}{x1.68} \\ \cline{6-11} 
 &  &  &  &  & GoogLeNet \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.60 & \multicolumn{2}{c|}{x1.16} \\ \cline{6-11} 
\multirow{-5}{*}{AQ'18} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 \footref{fc16}& \multicolumn{2}{c|}{FW32A} & 99.71 & \multicolumn{2}{c|}{x1.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ (or Computational) \footnote{When activations are quantized along with the weights, the computational savings are reported rather than model size savings}\\ Savings \footnote{\label{size}Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{} & 92.72 & \multicolumn{2}{c|}{x16.6} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-56 & \multicolumn{2}{c|}{} & 94.57 & \multicolumn{2}{c|}{x18.93} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-3}{*}{Cifar-10} & ResNet-110 & \multicolumn{2}{c|}{\multirow{-3}{*}{FW32A \footnote{\label{res1}Activations, the 1st and the last layer are kept in full precision}}} & 95.07 & \multicolumn{2}{c|}{x20.3} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 71.21 & \multicolumn{2}{c|}{x21.1} \\ \cline{7-11} 
 &  &  &  &  & \multirow{-2}{*}{ResNet-18 \footnote{\label{res3}ReLU-only preactivation}} & \multicolumn{2}{c|}{FWFA \footnote{\label{res2}1st and last layer are kept in full precision}} & 71.01 & \multicolumn{2}{c|}{x103.5} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 74.61 & \multicolumn{2}{c|}{x19.0} \\ \cline{7-11} 
\multirow{-8}{*}{DNAS'18} & \multirow{-8}{*}{DS} & \multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-8}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \multirow{-2}{*}{ResNet-34 \footref{res3}} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 74.21 & \multicolumn{2}{c|}{x87.4} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footnote{\label{accloss}Compared to the full precision model}\end{tabular} & \multicolumn{2}{c|}{Speedup \footnote{On conventional hardware using TVM compiler. Baseline: 8-bit precision models for inference}} \\ \cline{5-11} 
 &  &  &  & ImageNet & AlexNet & \multicolumn{2}{c|}{5W32A} & 0.08 & \multicolumn{2}{c|}{x3.95} \\ \cline{5-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{6.43W32A} & 0.26 & \multicolumn{2}{c|}{x1.24} \\ \cline{5-11} 
 &  &  &  &  & SimpleNet & \multicolumn{2}{c|}{5W32A} & 0.30 & \multicolumn{2}{c|}{x1.92} \\ \cline{6-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{2.81W32A} & 0.12 & \multicolumn{2}{c|}{x3.27} \\ \cline{6-11} 
 &  &  &  &  & VGG-11 & \multicolumn{2}{c|}{6.44W32A} & 0.17 & \multicolumn{2}{c|}{x1.53} \\ \cline{6-11} 
 &  &  &  & \multirow{-4}{*}{Cifar-10} & VGG-16 & \multicolumn{2}{c|}{7.25W32A} & 0.10 & \multicolumn{2}{c|}{-} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet & \multicolumn{2}{c|}{2.25W32A} & 0.00 & \multicolumn{2}{c|}{x2.76} \\ \cline{5-11} 
\multirow{-9}{*}{ReLeQ'18} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}LSTM-based\\ RL\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{None} & SVHN & SVHN-10 & \multicolumn{2}{c|}{4.8W32A} & 100 & \multicolumn{2}{c|}{x2.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{The weights of the output layer are left in full precision in experiments on CIFAR-10\/100 and Pascal VOC, and the weights of the input and output layers are left in full precision in the experiments on ImageNet}\end{tabular}} & \multicolumn{3}{c|}{Top-1\% Accuracy} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{W4A} & \multicolumn{3}{c|}{90.54} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-10} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{93.22} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{3.82W4A} & \multicolumn{3}{c|}{64.28} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-100} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{71.53} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{1.10W2A} & \multicolumn{3}{c|}{53.18} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{1.42W2A} & \multicolumn{3}{c|}{65.03} \\ \cline{5-11} 
 &  &  &  &  & SSD-300 & \multicolumn{2}{c|}{1.22W2A} & \multicolumn{3}{c|}{62.21} \\ \cline{6-11} 
\multirow{-9}{*}{PDB'19} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based on\\ input separability\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{Fixed} & \multirow{-2}{*}{Pascal VOC} & Faster R-CNN & \multicolumn{2}{c|}{1.52W4A} & \multicolumn{3}{c|}{74.52} \\ \hline
{\color[HTML]{000000} } &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
{\color[HTML]{000000} } &  &  &  & Cifar-10 \footnote{\label{memconst}Without constraints, and the networks are initialized with a pre-trained floating point network} & ResNet-20 \footnote{\label{uniform}With best parametrization of uniform DQ} & \multicolumn{2}{c|}{} & 92.60 & \multicolumn{2}{c|}{-} \\ \cline{5-6} \cline{9-11} 
{\color[HTML]{000000} } &  &  &  &  & MobileNet-V2 \footref{uniform} & \multicolumn{2}{c|}{} & 70.59 & \multicolumn{2}{c|}{x4.21} \\ \cline{6-6} \cline{9-11} 
\multirow{-4}{*}{{\color[HTML]{000000} DQ'19}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & \multirow{-2}{*}{ImageNet \footref{memconst}} & ResNet-18 \footref{uniform} & \multicolumn{2}{c|}{\multirow{-3}{*}{FWFW}} & 70.66 & \multicolumn{2}{c|}{x4.24} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Constraint\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Savings \footnote{Baseline: 8W8A models with energy and latency constraints, 32W32A models with model size constraint}\end{tabular} \\ \cline{5-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{edge}Edge Accelerator} & \multicolumn{2}{c|}{6.8W5.42A} & 70.58 &  & x1.66 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{cloud}Cloud Accelerator} & \multicolumn{2}{c|}{5.73W4.77A} & 69.97 &  & x1.95 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{bitfusion}BitFusion} & \multicolumn{2}{c|}{FWFA} & 70.40 &  & x1.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{edge} & \multicolumn{2}{c|}{5.86W6.10A} & 71.89 &  & x1.4 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{cloud} & \multicolumn{2}{c|}{4.92W5.29A} & 71.85 & \multirow{-5}{*}{Latency} & x1.45 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 \footref{bitfusion} & \multicolumn{2}{c|}{FWFA} & 70.37 & Energy & x1.9 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FWFA} & 71.74 &  & x7.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{3.85WFA} & 71.47 &  & x7.47 \\ \cline{6-9} \cline{11-11} 
\multirow{-10}{*}{HAQ'19} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}RL w/\\ budget constraints\end{tabular}} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding/\\ Vector Quant.\end{tabular}} & \multirow{-10}{*}{Mixed} & \multirow{-9}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 76.14 & \multirow{-3}{*}{Model Size} & x8.03 \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{w-s}In terms of weight compression. Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & Cifar-10 & ResNet-20 & \multicolumn{2}{c|}{4.05W4A \footnote{fixed 4 bits are used for activations in all layers except the 1st and last, where 8 bits are used}} & 92.22 & \multicolumn{2}{c|}{x13.11} \\ \cline{5-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{3.43W4.11A} & 75.52 & \multicolumn{2}{c|}{x12.04} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.48 & \multicolumn{2}{c|}{x12.28} \\ \cline{6-11} 
\multirow{-5}{*}{HAWQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hessian\\ Spectrum\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Fixed/Mixed} & \multirow{-3}{*}{ImageNet} & SqueezeNet & \multicolumn{2}{c|}{FWFA} & 68.02 & \multicolumn{2}{c|}{x9.25} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{\label{kernel}Kernel-wise quantization results are reported}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footnote{Baseline: 16W16F models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{3.32W4.12A} & 30.22 & \multicolumn{2}{c|}{x4.06} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4.02W3.93A} & 25.53 & \multicolumn{2}{c|}{x3.86} \\ \cline{6-11} 
 &  &  &  &  & SqueezeNet-V1 & \multicolumn{2}{c|}{3.76W4.05A} & 43.51 & \multicolumn{2}{c|}{x3.06} \\ \cline{6-11} 
\multirow{-5}{*}{AutoQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hierarchical\\ deep RL\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{3.67W4.14A} & 29.21 & \multicolumn{2}{c|}{xx3.42} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 \footnote{\label{1stlast}1st and last layer are kept in full precision} & \multicolumn{2}{c|}{FW32A} & 69.60 & \multicolumn{2}{c|}{x13.9} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{ImageNet} & MobileNet-V2 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 71.65 & \multicolumn{2}{c|}{x9.1} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 92.27 & \multicolumn{2}{c|}{x28.3} \\ \cline{6-11} 
 &  &  &  &  & ResNet-56 \footref{1stlast} \footnote{With cutout operation} & \multicolumn{2}{c|}{FW32A} & 94.48 & \multicolumn{2}{c|}{x23.2} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-10} & MobileNet-V2 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 93.28 & \multicolumn{2}{c|}{x12.4} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 68.18 & \multicolumn{2}{c|}{x11.6} \\ \cline{6-11} 
 &  &  &  &  & Res-Net-56 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 71.84 & \multicolumn{2}{c|}{x17.2} \\ \cline{6-11} 
\multirow{-9}{*}{CBAQ'19} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Cursor-based\\ DS \end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-9}{*}{None} & \multirow{-3}{*}{CIFAR-100} & MobileNet-V2 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 68.04 & \multicolumn{2}{c|}{x12.9} \\ \hline
 \end{tabular}%
}
%\afterpage{\clearpage}
\end{table}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\
\hline
  &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ Savings \footnote{\label{mbnet}Baseline: 8-bit precision quantized MobileNet-V2}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footref{mbnet}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-100 & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 68.38 & x3.26 & x3.49 \\ \cline{5-11} 
\multirow{-3}{*}{MPNASEE'19} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ \\ energy constraints\\ and a proxy task\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 77.84 & x5.09 & x5.19 \\ \hline
&  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Giga Bit\\ Operation \\ Count Savings \footnote{Of full precision model}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet-5 & \multicolumn{2}{c|}{FWFA} & 99.30 & \multicolumn{2}{c|}{x277.78} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & VGG-7 & \multicolumn{2}{c|}{FWFA} & 93.23 & \multicolumn{2}{c|}{x196.08} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 69.36 & \multicolumn{2}{c|}{x51.81} \\ \cline{6-11} 
\multirow{-5}{*}{Bayesian Bits'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Variational\\ inference\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{FWFA} & 72 & \multicolumn{2}{c|}{x16} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top 1-\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Bit Operations\\ Savings \footnote{Baseline: 4W4A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 \footnote{\label{res-blocks}Only res-blocks are searched and quantized; excluding the 1st convolution layer and last fully connected layer} & \multicolumn{2}{c|}{FWFA} & 70.50 & \multicolumn{2}{c|}{x1.04} \\ \cline{6-11} 
\multirow{-3}{*}{SPOSNAS'20} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}ES w/ budget\\ constraints\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & ResNet-34 \footref{res-blocks} & \multicolumn{2}{c|}{FWFA} & 74.60 & \multicolumn{2}{c|}{x1.02} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top 1-\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Bit Operations\\ Savings \footref{mbnet}\end{tabular}} \\ \cline{5-11} 
\multirow{-3}{*}{APQ'20} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Predictor-based\\ES w/ budget\\ constraints\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Their joint designed models & \multicolumn{2}{c|}{FWFA} & 75.1 & \multicolumn{2}{c|}{x1.23} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy (or mAP) \footnote{mAP is used for COCO dataset}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bit Operations\\ Budget\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{4W3.9A} & 92.30 & 4 & x10.19 \\ \cline{5-11} 
 &  &  &  & ImageNet & ResNet-50 & \multicolumn{2}{c|}{-} & 76.67 & 4 & - \\ \cline{5-11} 
\multirow{-4}{*}{BP-NAS'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ complexity\\ constraints\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining \\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & Microsoft COCO & \begin{tabular}[c]{@{}c@{}}ResNet-50 \\ (faster R-CNN)\end{tabular} & \multicolumn{2}{c|}{3.84W4.31A} & 0.358 & 4 & - \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Memory\\ Savings \footnote{Baseline: XNOR network}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footnote{\label{identity}With identity shortcut connections at each layer} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.88 & \multicolumn{2}{c|}{0.53} \\ \cline{6-11} 
 &  &  &  &  & ResNet-32 \footref{identity} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 64.45 & \multicolumn{2}{c|}{0.69} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-100} & VGG-15 & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.38 & \multicolumn{2}{c|}{0.50} \\ \cline{5-11} 
\multirow{-5}{*}{Hybrid-Net'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based\\ on PCA\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & ImageNet & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 62.73 & \multicolumn{2}{c|}{0.80} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 92.43 & \multicolumn{2}{c|}{x11.06} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.45 & \multicolumn{2}{c|}{x13.1} \\ \cline{6-11} 
 &  &  &  &  & EfficientNet-B0 & \multicolumn{2}{c|}{FW8A} & 74.6 & \multicolumn{2}{c|}{x11.97} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FW8A} & 69.88 & \multicolumn{2}{c|}{x10.68} \\ \cline{6-11} 
\multirow{-6}{*}{HMQ'20} & \multirow{-6}{*}{DS} & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-6}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{FWFA} & 70.9 & \multicolumn{2}{c|}{x8.05} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{Using efficient composite convolution with respect to vanilla parallel convolutions}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{AlexNet} & \multicolumn{2}{c|}{2W2A} & 59.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{-}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 68 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & 67 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-18} & \multicolumn{2}{c|}{2W2A} & 65.9 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{GoogLeNet} & \multicolumn{2}{c|}{2W2A} & 67.8 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.45}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-50} & \multicolumn{2}{c|}{2W2A} & 72.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
\multirow{-16}{*}{EdMIPS'20} & \multirow{-16}{*}{DS} & \multirow{-16}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-16}{*}{Mixed} & \multirow{-15}{*}{ImageNet} & \multirow{-3}{*}{Inception-V3} & \multicolumn{2}{c|}{2W2A} & 72.4 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{size}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{} & 77.43 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{} & 72.85 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ShuffleNet & \multicolumn{2}{c|}{} & 62.90 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-152 & \multicolumn{2}{c|}{} & 77.88 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{} & 78.76 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & SqueezeNext & \multicolumn{2}{c|}{} & 68.17 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-7}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{} & 71.30 & \multicolumn{2}{c|}{x5.34} \\ \cline{5-6} \cline{9-11} 
 &  &  &  & Cifar-10 & ResNet-20 & \multicolumn{2}{c|}{} & 93.87 & \multicolumn{2}{c|}{x5.20} \\ \cline{5-6} \cline{9-11} 
\multirow{-10}{*}{ZeroQ'20} & \multirow{-10}{*}{Pareto Frontier} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-10}{*}{Fixed} & Microsoft COCO & RetinaNet & \multicolumn{2}{c|}{\multirow{-9}{*}{FW6A}} & 35.9 & \multicolumn{2}{c|}{x6.00} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy \footnote{Reported for EBS with deterministic search}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Computational\\ Savings \footnote{In terms of FLOPs}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{FWFA} & 92.94 & \multicolumn{2}{c|}{x4.01} \\ \cline{6-11} 
 &  &  &  &  & ResNet-32 & \multicolumn{2}{c|}{FWFA} & 93.53 & \multicolumn{2}{c|}{x3.24} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-10} & ResNet-56 & \multicolumn{2}{c|}{FWFA} & 94.27 & \multicolumn{2}{c|}{x3.76} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 70.20 & \multicolumn{2}{c|}{x3.26} \\ \cline{6-11} 
\multirow{-6}{*}{EBS'20} & \multirow{-6}{*}{DS} & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-6}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & ResNet-34 & \multicolumn{2}{c|}{FWFA} & 73.50 & \multicolumn{2}{c|}{x3.33} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet5 \footnote{Based on \cite{}} & \multicolumn{2}{c|}{-} & 99.12 & \multicolumn{2}{c|}{x75.77} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & VGG \footnote{Based on \cite{}} & \multicolumn{2}{c|}{0.66W32A} & 92.00 & \multicolumn{2}{c|}{x43.48} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{2W32A} & 68.90 & \multicolumn{2}{c|}{x13.58} \\ \cline{6-11} 
\multirow{-5}{*}{ALQ'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Vector Quant.\end{tabular}} & \multirow{-5}{*}{Fixed/None} & \multirow{-2}{*}{ImageNet} & ResNet-34 & \multicolumn{2}{c|}{2W2A} & 71.00 & \multicolumn{2}{c|}{x13.68} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footref{accloss}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{bl}Baseline: 32W32F}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.30} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.10} \\ \cline{6-11} 
\multirow{-4}{*}{ADRL'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Deep RL w/\\ compression\\ ratio constraint\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{None} & \multirow{-2}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.00} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \multicolumn{3}{c|}{Top-1\% Accuracy \footnote{Random per layer bit selection}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{65.8} \\ \cline{6-11} 
 &  &  &  &  & ResNet-34 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{70.5} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{73.2} \\ \cline{6-11} 
\multirow{-5}{*}{Bit-Mixer'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}3-stage\\ optimization on\\ Meta-Network\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \begin{tabular}[c]{@{}c@{}}EBN \\ 4:4:4:4\end{tabular} & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{72.1} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{2.99W32A} & 57.09 & \multicolumn{2}{c|}{x138.96} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 & \multicolumn{2}{c|}{2.92W32A} & 71.39 & \multicolumn{2}{c|}{x195.87} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{3.26W32A} & 70.83 & \multicolumn{2}{c|}{x23.26} \\ \cline{6-11} 
\multirow{-5}{*}{OPQ'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Codebook\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{3.25W32A} & 76.41 & \multicolumn{2}{c|}{x38.03} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{bl}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{FW4A \footnote{\label{activate}First and last layer activations are left as 8-bit precision}} & 92.32 & \multicolumn{2}{c|}{x14.24} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FW4A \footref{activate}} & 75.29 & \multicolumn{2}{c|}{x11.90} \\ \cline{6-11} 
\multirow{-4}{*}{BSQ'21} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Fixed} & \multirow{-2}{*}{ImageNet} & Inception-V3 & \multicolumn{2}{c|}{FW6A} & 76.60 & \multicolumn{2}{c|}{x11.38} \\ \hline
\end{tabular}
}
\end{table}

==> Mixed Precision Frameworks Survey/test.tex <==
\begin{landscape}
\begin{figure}
\vspace{-1cm}
\centering
\begin{tikzpicture}
\path[mindmap,concept color=black,text=white]
    node[concept] {Mixed Precision\\ Frameworks}
    [clockwise from=140]
    
    child[concept color=orange, yshift=-3.5cm, grow=-180,font=\fontsize{10pt}{16pt}]{ 
        node[concept] {Gradient-Based\\Optimization}
            [clockwise from=-60]
        % child {node[concept] {\cite{}} }
        child {node[concept] {SLWP(\cite{lacey2018stochastic})} }
        child {node[concept] {DQ (\cite{uhlich2019differentiable})} }
        child {node[concept] {Bayesian Bits (\cite{van2020bayesian})}
        }}
    child[concept  color=orange, grow=-90, xshift=2cm,] 
    { 
        node[concept] {Heuristic-Based\\Optimization}
            [clockwise from=-40]
        % child {node[concept] {\cite{}} }
        child {node[concept] {AQ(\cite{zhou2018adaptive})} }
        child {node[concept] {PDB (\cite{chu2019mixed})} }
        child {node[concept] {HAWQ (\cite{dong2019hawq})}}
        child {node[concept] {Hybrid-Net (\cite{chakraborty2020constructing})}}  
        child {node[concept] {ZeroQ (\cite{cai2020zeroq})}}
        child {node[concept] {OPQ (\cite{hu2021opq})}
        } }
    child[concept  color=orange, grow=10, xshift=2cm,font=\fontsize{10pt}{16pt}]
    { 
        node[concept] {Meta-Heuristic-Based\\Optimization}
            [clockwise from=-90]
        child {node[concept]{DNAS (\cite{wu2018mixed})} }
        child {node[concept] {MPNASEE (\cite{pan2019})} }
        child {node[concept] {APQ (\cite{wang2020apq})}}
        child {node[concept] {BP-NAS (\cite{yu2020search})}}
        child {node[concept] {HMQ (\cite{habi2020hmq})}}
        child {node[concept] {EdMIPS (\cite{cai2020rethinking})}}
        child {node[concept] {Bit-Mixer (\cite{bulat2021bit})}}
        };
\end{tikzpicture}
\label{mindmap}
\caption{Alternative approaches and different methods for approximating a CPE}
\end{figure}
\end{landscape}
 
 
\begin{comment}

\begin{tikzpicture}
\path[mindmap,concept color=black,text=white]
    node[concept] {Constant Phase\\ Element}
    [clockwise from=140]
    child[concept  color=orange, grow=-20, xshift=2cm,] { 
     node[concept  ,scale=1.5,font=\fontsize{10pt}{20pt}] {Emulators}
        child [concept color=black!40, grow=-170]{node[concept, scale=1.5,yshift=-2cm] {TF based Approx.}  
        [clockwise from=-110]
            child {node[concept,scale=1.5,yshift=-0.8cm] {Oustaloup\\ \cite{oustaloup1996crone} }}
            child {node[concept,scale=1.5,xshift=-0.6cm,yshift=-0.7cm] {Matsuda\\ \cite{khoichi1993h}} }
            child {node[concept,scale=1.5,xshift=-1cm,yshift=-0.4cm] {CFE\\ \cite{roy1967realization}}}
            child {node[concept,scale=1.5,xshift=-1cm,yshift=0.1cm] {Charef\\ \cite{charef1992fractal}} }
            child {node[concept,scale=1.5,xshift=-0.5cm,yshift=0.4cm] {Carlson\\ \cite{carlson1960simulation}} } }
        child [concept color=black!40, grow=-30] {node[concept,scale=1.5, xshift=1.5cm] {Circuit Inspired Approx.}
            child[concept color=red!60!black, grow=-90] {node[concept,scale=2, yshift=-1.5cm ] {Systematic \\ Synthesis}
            [clockwise from=60]
            child {node[concept,scale=2,xshift=0.5cm,yshift=0.5cm] {Valsa\\ \cite{valsa2011network} }}
            child {node[concept,scale=2,xshift=0.7cm,yshift=-0.2cm] {Morrison\\ \cite{morrison1959rc}} }
            child {node[concept,scale=2,xshift=0.3cm,yshift=-1.cm] {Sugi \\ \cite{sugi2002frequency}} } }
            child [concept color=yellow!60!black, grow=-135] {node[concept, scale=2, xshift=-1.2cm,yshift=-2.5cm] {Optimization} 
            [clockwise from=-30]
                child {node[concept,scale=2, xshift=0.7cm ] {Yousri\\ \cite{YOUSRI2019110}} }
                child {node[concept,scale=2, xshift=0, yshift=-0.7cm ] {Oshakov\\ \cite{ARKHIPOVICHUSHAKOV2020}} }
                child {node[concept,scale=2, xshift=-0.7cm, yshift=-0.7cm ] {Kartci \cite{kartci2019synthesis}} }
                child [concept color=green!60!blue] {node[concept,scale=2, xshift=-1cm, yshift=0cm ] {This \\ Work} }
            }
    }}
    child[concept color=orange, yshift=-3.5cm, grow=180,font=\fontsize{10pt}{16pt}]{ 
        node[concept] {Fabrication}
            [clockwise from=-60]
        % child {node[concept] {\cite{}} }
        child {node[concept] {Fractal structure  \cite{jesus2009development,598289,haba2005influence}} }
        child {node[concept] {polymers \cite{caponetto2013experimental,agambayev2018ultra}} }
        child {node[concept] {Solid-state \cite{BUSCARINO2018307,john2017solid,adhikary2015realization,elshurafa2013microscale}} }
        child {node[concept] {Electro-chemical \cite{1705043,6262466}} }
    };
\end{tikzpicture}
\label{mindmap}
\caption{Alternative approaches and different methods for approximating a CPE}

\end{comment}

==> Mixed Precision Frameworks Survey/tree.tex <==
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white,
                     bottom color=blue!20},
  root/.style     = {treenode, font=\Large,
                     bottom color=red!30},
  env/.style      = {treenode, font=\ttfamily\normalsize},
  dummy/.style    = {circle,draw},
}

\begin{figure}
\centering
\begin{tikzpicture}   [
    grow                    = right,
    level distance          = 10em,
    edge from parent/.style = {draw, -latex},
    every node/.style       = {font=\footnotesize},
    sloped,
    level 1/.style={sibling distance=63mm},level 2/.style={sibling distance=21.9mm},level 3/.style={sibling distance=5.5mm}
  ]

\node [root] {MXPDNN\\Framework}
	child {node [env] {Meta-heurisric-based\\Optimization}
	child {node [env] {Retraining}
	child {node [env] {Bit-Mixer \cite{bulat2021bit}}}
	child {node [env] {HMQ \cite{habi2020hmq}}}
	child {node [env] {BP-NAS \cite{yu2020search}}}
	child {node [env] {APQ \cite{wang2020apq}}}
	child {node [env] {DNAS \cite{wu2018mixed}}}
	}
	child {node [env] {Post-training}
	child {node [env] {EvoQ\cite{evoq}}}
	child {node [env] {JASQ\cite{chen2018joint}}}
	}
	child {node [env] {Training-aware}
	child {node [env] {EdMIPS \cite{cai2020rethinking}}}
	child {node [env] {MPNASEE \cite{gong2019differentiable}}}
	}
	}
	child {node [env] {Heuristic-based\\Optimization}
	child {node [env] {Retraining}
	child {node [env] {MPQNNCO \cite{chen2021towards}}}
	child {node [env] {OPQ \cite{hu2021opq}}}
	child {node [env] {HAWQ-V3 \cite{yao2021hawq}}}
	child {node [env] {HAWQ-V2 \cite{dong2019hawq}}}
	}
	child {node [env] {Post-training}
	child {node [env] {ZeroQ \cite{cai2020zeroq}}}
	child {node [env] {HAWQ-V3 \cite{yao2021hawq}}}
	child {node [env] {Hybrid-Net \cite{chakraborty2020constructing}}}
	child {node [env] {AQ \cite{zhou2018adaptive}}}
	}
	child {node [env] {Training-aware}
	child {node [env] {PDB \cite{chu2019mixed}}}
	}
	}
	child {node [env] {RL-based\\Optimization}
	child {node [env] {Retraining}
	child {node [env] {ADRL \cite{ning2020simple}}}
	child {node [env] {AutoQ}}
	child {node [env] {HAQ \cite{wang2019haq}}}
	child {node [env] {ReLeQ \cite{elthakeb2018releq}}}
	}
	}
	child {node [env] {Gradient-based\\Optimization}
	child {node [env] {Retraining}
	child {node [env] {Bayesian Bits \cite{van2020bayesian}}}
	child {node [env] {DQ \cite{uhlich2019differentiable}}}
	child {node [env] {SLWP \cite{lacey2018stochastic}}}
	}
	child {node [env] {Post-training}
	child {node [env] {OBACWA \cite{zhe2019optimizing}}}
	}
	};

\end{tikzpicture}
\caption{Mixed Precision Frameworks grouped according to their optimization and quantization techniques.}
\label{mxdpdnn}
\end{figure}


==> Summary_Fig.tex <==
%\begin{landscape}
\begin{figure}
\centering
\begin{tikzpicture}
\path[mindmap,concept color=black,text=white,level 2 concept/.append style=
      {every child/.style={concept color=blue!70},sibling angle=-42}]
      
    node[concept] {Mixed Precision\\ Frameworks}
    [clockwise from=140]
    
    child[concept color=orange, yshift=-6cm, xshift=2.5cm grow=90,font=\fontsize{10pt}{16pt}]{ 
        node[concept] {Gradient-Based\\Optimization}
            [clockwise from=130]
        % child {node[concept] {\cite{}} }
        child {node[concept] {SLWP(\cite{lacey2018stochastic})} }
        child {node[concept] {DQ (\cite{uhlich2019differentiable})} }
        child {node[concept] {OBACWA (\cite{zhe2019optimizing})} }
        child {node[concept, xshift=5] {Bayesian Bits (\cite{van2020bayesian})}
        }}
    child[concept  color=orange, grow=-90, xshift=2cm] 
    { 
        node[concept] {Heuristic-Based\\Optimization}
            [clockwise from=170]
        % child {node[concept] {\cite{}} }
        child {node[concept] {AQ(\cite{zhou2018adaptive})} }
        child {node[concept] {PDB (\cite{chu2019mixed})} }
        child {node[concept] {HAWQ (\cite{dong2019hawq})}}
        child {node[concept] {HAWQ-V3 (\cite{yao2021hawq})}}
        child {node[concept] {Hybrid-Net (\cite{chakraborty2020constructing})}}  
        child {node[concept] {ZeroQ (\cite{cai2020zeroq})}}
        child {node[concept] {HAWQ-V3 (\cite{yao2021hawq})}}
        child {node[concept] {MPQNNCO (\cite{chen2021towards})}}
        child {node[concept] {OPQ (\cite{hu2021opq})}
        } }
    child[concept  color=orange, grow=0 xshift=3.5cm,yshift=3cm]
    { 
        node[concept] {Meta-Heuristic-Based\\Optimization}
            [clockwise from=63]
        child {node[concept]{DNAS (\cite{wu2018mixed})} }
        child {node[concept]{JASQ (\cite{chen2018joint})} }
        child {node[concept] {MPNASEE (\cite{pan2019})} }
        child {node[concept] {APQ (\cite{wang2020apq})}}
        child {node[concept, xshift=5] {BP-NAS (\cite{yu2020search})}}
        child {node[concept, yshift=-7] {HMQ (\cite{habi2020hmq})}}
        child {node[concept] {EdMIPS (\cite{cai2020rethinking})}}
        child {node[concept, yshift=4] {EvoQ (\cite{evoq})}}
        child {node[concept, xshift=40, grow=20, yshift=7] {Bit-Mixer (\cite{bulat2021bit})}}}
    child[concept  color=orange, grow=130, xshift=3.5cm,yshift=0.5cm]
    { 
        node[concept] {RL-Based\\Optimization}
            [clockwise from=60]
        child {node[concept, yshift=-15, xshift=10]{ReLeQ (\cite{elthakeb2018releq})} }
        child {node[concept] {HAQ (\cite{wang2019haq})} }
        child {node[concept] {AutoQ (\cite{lou2019autoq})}}
        child {node[concept] {ADRL (\cite{ning2020simple})}}
};
\end{tikzpicture}
\caption{Mixed Precision Frameworks grouped according to their optimization techniques.}
\label{mxdpdnn}
\end{figure}
%\end{landscape}
 
 

==> Table_inter.tex <==
\begin{table}[]
\centering
\caption{Summary of Mixed Precision Frameworks, where at least weights are quantized with mixed bit precision. In "XWYA", "XW" and "YA" stand for the (average) \# of bits of weights and activations respectively. "X"/"Y"="F" when "W"/"A" take "Flexible" precision assignments layer-wise. "QOP"=quantization as an optimization problem. "DS"=Differentiable Search. "ES"=Evolutionary Search.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Precision Budget\\ (in bits)\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 97.68 & \multicolumn{2}{c|}{10} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 98.31 & \multicolumn{2}{c|}{20} \\ \cline{7-11} 
 &  &  &  & \multirow{-3}{*}{MNIST} & \multirow{-3}{*}{Similar to LeNet-5} & \multicolumn{2}{c|}{8W8A} & 98.86 & \multicolumn{2}{c|}{40} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 51.46 & \multicolumn{2}{c|}{14} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 52.31 & \multicolumn{2}{c|}{28} \\ \cline{7-11} 
\multirow{-7}{*}{SLWP'18} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Gradient-Based\end{tabular}} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-7}{*}{Mixed} & \multirow{-3}{*}{ImageNet} & \multirow{-3}{*}{AlexNet \footnote{1st layer is kept in full precision}} & \multicolumn{2}{c|}{8W8A} & 52.54 & \multicolumn{2}{c|}{56} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\% \\Accuracy \end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\Savings \footnote{Baseline: Equal bit-width quantized models across all layers}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet \footnote{\label{fc16}Fully connected layers are kept in 16-bit precision} & \multicolumn{2}{c|}{FW32A} & 99.50 & \multicolumn{2}{c|}{x1.84} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.68 & \multicolumn{2}{c|}{x1.68} \\ \cline{6-11} 
 &  &  &  &  & GoogLeNet \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.60 & \multicolumn{2}{c|}{x1.16} \\ \cline{6-11} 
\multirow{-5}{*}{AQ'18} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 \footref{fc16}& \multicolumn{2}{c|}{FW32A} & 99.71 & \multicolumn{2}{c|}{x1.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ (or Computational) \footnote{When activations are quantized along with the weights, the computational savings are reported rather than model size savings}\\ Savings \footnote{\label{size}Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{} & 92.72 & \multicolumn{2}{c|}{x11.6} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-56 & \multicolumn{2}{c|}{} & 94.57 & \multicolumn{2}{c|}{x14.6} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-10} & ResNet-110 & \multicolumn{2}{c|}{\multirow{-3}{*}{FW32A \footnote{\label{res1}Activations, the 1st and the last layer are kept in full precision}}} & 95.07 & \multicolumn{2}{c|}{x12.5} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 71.21 & \multicolumn{2}{c|}{x11.2} \\ \cline{7-11} 
 &  &  &  &  & \multirow{-2}{*}{ResNet-18 \footnote{\label{res3}ReLU-only preactivation}} & \multicolumn{2}{c|}{FWFA \footnote{\label{res2}1st and last layer are kept in full precision}} & 71.01 & \multicolumn{2}{c|}{x33.2} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 74.61 & \multicolumn{2}{c|}{x10.6} \\ \cline{7-11} 
\multirow{-8}{*}{DNAS'18} & \multirow{-8}{*}{DS} & \multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-8}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \multirow{-2}{*}{ResNet-34 \footref{res3}} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 74.21 & \multicolumn{2}{c|}{x40.8} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footnote{\label{accloss}Compared to the full precision model}\end{tabular} & \multicolumn{2}{c|}{Speedup \footnote{On conventional hardware using TVM compiler. Baseline: 8-bit precision models for inference}} \\ \cline{5-11} 
 &  &  &  & \multirow{2}{*}{ImageNet} & AlexNet & \multicolumn{2}{c|}{5W32A} & 0.08 & \multicolumn{2}{c|}{x3.95} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{6.43W32A} & 0.26 & \multicolumn{2}{c|}{x1.24} \\ \cline{5-11} 
 &  &  &  &  & SimpleNet & \multicolumn{2}{c|}{5W32A} & 0.30 & \multicolumn{2}{c|}{x1.92} \\ \cline{6-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{2.81W32A} & 0.12 & \multicolumn{2}{c|}{x3.27} \\ \cline{6-11} 
 &  &  &  &  & VGG-11 & \multicolumn{2}{c|}{6.44W32A} & 0.17 & \multicolumn{2}{c|}{x1.53} \\ \cline{6-11} 
 &  &  &  & \multirow{-4}{*}{CIFAR-10} & VGG-16 & \multicolumn{2}{c|}{7.25W32A} & 0.10 & \multicolumn{2}{c|}{-} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet-5 & \multicolumn{2}{c|}{2.25W32A} & 0.00 & \multicolumn{2}{c|}{x2.76} \\ \cline{5-11} 
\multirow{-9}{*}{ReLeQ'18} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}LSTM-based\\ RL\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{None} & SVHN & SVHN-10 & \multicolumn{2}{c|}{4.8W32A} & 100 & \multicolumn{2}{c|}{x2.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{The weights of the output layer are left in full precision in experiments on CIFAR-10\/100 and Pascal VOC, and the weights of the input and output layers are left in full precision in the experiments on ImageNet}\end{tabular}} & \multicolumn{3}{c|}{Top-1\% Accuracy} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{W4A} & \multicolumn{3}{c|}{90.54} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-10} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{93.22} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{3.82W4A} & \multicolumn{3}{c|}{64.28} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-100} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{71.53} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{1.10W2A} & \multicolumn{3}{c|}{53.18} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{1.42W2A} & \multicolumn{3}{c|}{65.03} \\ \cline{5-11} 
 &  &  &  &  & SSD-300 & \multicolumn{2}{c|}{1.22W2A} & \multicolumn{3}{c|}{62.21} \\ \cline{6-11} 
\multirow{-9}{*}{PDB'19} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based on\\ input separability\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{Fixed} & \multirow{-2}{*}{Pascal VOC} & Faster R-CNN & \multicolumn{2}{c|}{1.52W4A} & \multicolumn{3}{c|}{74.52} \\ \hline
{\color[HTML]{000000} } &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
{\color[HTML]{000000} } &  &  &  & CIFAR-10 \footnote{\label{memconst}Without constraints, and the networks are initialized with a pre-trained floating point network} & ResNet-20 \footnote{\label{uniform}With best parametrization of uniform DQ} & \multicolumn{2}{c|}{} & 92.60 & \multicolumn{2}{c|}{-} \\ \cline{5-6} \cline{9-11} 
{\color[HTML]{000000} } &  &  &  &  & MobileNet-V2 \footref{uniform} & \multicolumn{2}{c|}{} & 70.59 & \multicolumn{2}{c|}{x4.21} \\ \cline{6-6} \cline{9-11} 
\multirow{-4}{*}{{\color[HTML]{000000} DQ'19}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Gradient-Based\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & \multirow{-2}{*}{ImageNet \footref{memconst}} & ResNet-18 \footref{uniform} & \multicolumn{2}{c|}{\multirow{-3}{*}{FWFW}} & 70.66 & \multicolumn{2}{c|}{x4.24} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Constraint\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Savings \footnote{Baseline: 8W8A models with energy and latency constraints, 32W32A models with model size constraint}\end{tabular} \\ \cline{5-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{edge}Edge Accelerator} & \multicolumn{2}{c|}{6.8W5.42A} & 70.58 &  & x1.66 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{cloud}Cloud Accelerator} & \multicolumn{2}{c|}{5.73W4.77A} & 69.97 &  & x1.95 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{bitfusion}BitFusion} & \multicolumn{2}{c|}{FWFA} & 70.40 &  & x1.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{edge} & \multicolumn{2}{c|}{5.86W6.10A} & 71.89 &  & x1.4 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{cloud} & \multicolumn{2}{c|}{4.92W5.29A} & 71.85 & \multirow{-5}{*}{Latency} & x1.45 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 \footref{bitfusion} & \multicolumn{2}{c|}{FWFA} & 70.37 & Energy & x1.9 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FWFA} & 71.74 &  & x7.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{3.85WFA} & 71.47 &  & x7.47 \\ \cline{6-9} \cline{11-11} 
\multirow{-10}{*}{HAQ'19} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}RL w/\\ budget constraints\end{tabular}} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\\ Vector Quant.\end{tabular}} & \multirow{-10}{*}{Mixed} & \multirow{-9}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 76.14 & \multirow{-3}{*}{Model Size} & x8.03 \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{w-s}In terms of weight compression. Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{4.05W4A \footnote{fixed 4 bits are used for activations in all layers except the 1st and last, where 8 bits are used}} & 92.22 & \multicolumn{2}{c|}{x13.11} \\ \cline{5-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{3.43W4.11A} & 75.52 & \multicolumn{2}{c|}{x12.04} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.48 & \multicolumn{2}{c|}{x12.28} \\ \cline{6-11} 
\multirow{-5}{*}{HAWQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hessian\\ Spectrum\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Fixed/Mixed} & \multirow{-3}{*}{ImageNet} & SqueezeNet & \multicolumn{2}{c|}{FWFA} & 68.02 & \multicolumn{2}{c|}{x9.25} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{\label{kernel}Kernel-wise quantization results are reported}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy \footnote{Resource-constrained experiments}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footnote{Baseline: 16W16F models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{3.32W4.12A} & 69.78 & \multicolumn{2}{c|}{x4.06} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4.02W3.93A} & 74.47 & \multicolumn{2}{c|}{x3.86} \\ \cline{6-11} 
 &  &  &  &  & SqueezeNet-V1 & \multicolumn{2}{c|}{3.76W4.05A} & 56.49 & \multicolumn{2}{c|}{x3.06} \\ \cline{6-11} 
\multirow{-5}{*}{AutoQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hierarchical\\ deep RL\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{3.67W4.14A} & 70.79 & \multicolumn{2}{c|}{x3.43} \\  \hline
 \end{tabular}%
}
%\afterpage{\clearpage}
\end{table}


\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\
\hline
  &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ Savings \footnote{\label{mbnet}Baseline: 8-bit precision quantized MobileNet-V2}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footref{mbnet}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-100 & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 68.38 & x3.26 & x3.49 \\ \cline{5-11} 
\multirow{-3}{*}{MPNASEE'19} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ \\ energy constraints\\ and a proxy task\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 77.84 & x5.09 & x5.19 \\ \hline
&  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Giga Bit\\ Operation \\ Count Savings \footnote{Of full precision model}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet-5 \footnote{\label{logit}Output logits left in full precision}& \multicolumn{2}{c|}{FWFA} & 99.30 & \multicolumn{2}{c|}{x277.78} \\ \cline{5-11} 
 &  &  &  & CIFAR-10  & VGG-7 \footref{logit}& \multicolumn{2}{c|}{FWFA} & 93.23 & \multicolumn{2}{c|}{x196.08} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 \footref{logit}& \multicolumn{2}{c|}{FWFA} & 69.36 & \multicolumn{2}{c|}{x51.81} \\ \cline{6-11} 
\multirow{-5}{*}{Bayesian Bits'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Variational\\ inference\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & MobileNet-V2 \footref{logit}& \multicolumn{2}{c|}{FWFA} & 72 & \multicolumn{2}{c|}{x16} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top 1-\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Bit Operations\\ Savings \footnote{Baseline: 4W4A models}\end{tabular}} \\ \cline{5-11} 
\multirow{-3}{*}{APQ'20} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Predictor-based\\ES w/ budget\\ constraints\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Their model & \multicolumn{2}{c|}{FWFA} & 75.1 & \multicolumn{2}{c|}{x1.23} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy (or mAP) \footnote{mAP is used for COCO dataset}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bit Operations\\ Budget\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{4W3.9A} & 92.30 & 4 & x10.19 \\ \cline{5-11} 
 &  &  &  & ImageNet & ResNet-50 & \multicolumn{2}{c|}{-} & 76.67 & 4 & - \\ \cline{5-11} 
\multirow{-4}{*}{BP-NAS'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ complexity\\ constraints\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining \\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & Microsoft COCO & \begin{tabular}[c]{@{}c@{}}ResNet-50 \\ (faster R-CNN)\end{tabular} & \multicolumn{2}{c|}{3.84W4.31A} & 0.358 & 4 & - \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\%Degradation\\ Memory\\ Compression \footnote{Baseline: XNOR network}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footnote{\label{identity}With identity shortcut connections at each layer} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.88 & \multicolumn{2}{c|}{47} \\ \cline{6-11} 
 &  &  &  &  & ResNet-32 \footref{identity} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 64.45 & \multicolumn{2}{c|}{31} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-100} & VGG-15 & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.38 & \multicolumn{2}{c|}{50} \\ \cline{5-11} 
\multirow{-5}{*}{Hybrid-Net'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based\\ on PCA\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & ImageNet & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 62.73 & \multicolumn{2}{c|}{20} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 92.43 & \multicolumn{2}{c|}{x11.06} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.45 & \multicolumn{2}{c|}{x13.1} \\ \cline{6-11} 
 &  &  &  &  & EfficientNet-B0 & \multicolumn{2}{c|}{FW8A} & 74.6 & \multicolumn{2}{c|}{x11.97} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FW8A} & 69.88 & \multicolumn{2}{c|}{x10.68} \\ \cline{6-11} 
\multirow{-6}{*}{HMQ'20} & \multirow{-6}{*}{DS} & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-6}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{FWFA} & 70.9 & \multicolumn{2}{c|}{x8.05} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{Using efficient composite convolution with respect to vanilla parallel convolutions}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{AlexNet} & \multicolumn{2}{c|}{2W2A} & 59.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{-}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 68 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & 67 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-18} & \multicolumn{2}{c|}{2W2A} & 65.9 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{GoogLeNet} & \multicolumn{2}{c|}{2W2A} & 67.8 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.45}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-50} & \multicolumn{2}{c|}{2W2A} & 72.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
\multirow{-16}{*}{EdMIPS'20} & \multirow{-16}{*}{DS} & \multirow{-16}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-16}{*}{Mixed} & \multirow{-15}{*}{ImageNet} & \multirow{-3}{*}{Inception-V3} & \multicolumn{2}{c|}{2W2A} & 72.4 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{size}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{} & 77.43 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{} & 72.85 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ShuffleNet & \multicolumn{2}{c|}{} & 62.90 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-152 & \multicolumn{2}{c|}{} & 77.88 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{} & 78.76 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & SqueezeNext & \multicolumn{2}{c|}{} & 68.17 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-7}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{} & 71.30 & \multicolumn{2}{c|}{x5.34} \\ \cline{5-6} \cline{9-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{} & 93.87 & \multicolumn{2}{c|}{x5.20} \\ \cline{5-6} \cline{9-11} 
\multirow{-10}{*}{ZeroQ'20} & \multirow{-10}{*}{Pareto Frontier} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-10}{*}{Fixed} & Microsoft COCO & RetinaNet & \multicolumn{2}{c|}{\multirow{-9}{*}{FW6A}} & 35.9 & \multicolumn{2}{c|}{x6.00} \\ \hline
 

 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footref{accloss}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{bl}Baseline: 32W32F}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.30} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.10} \\ \cline{6-11} 
\multirow{-4}{*}{ADRL'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Deep RL w/\\ compression\\ ratio constraint\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{None} & \multirow{-2}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.00} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \multicolumn{3}{c|}{Top-1\% Accuracy \footnote{Random per layer bit selection}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{65.8} \\ \cline{6-11} 
 &  &  &  &  & ResNet-34 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{70.5} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{73.2} \\ \cline{6-11} 
\multirow{-5}{*}{Bit-Mixer'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}3-stage\\ optimization on\\ Meta-Network\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \begin{tabular}[c]{@{}c@{}}EBN \\ 4:4:4:4\end{tabular} & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{72.1} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{2.99W32A} & 57.09 & \multicolumn{2}{c|}{x138.96} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 & \multicolumn{2}{c|}{2.92W32A} & 71.39 & \multicolumn{2}{c|}{x195.87} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{3.26W32A} & 70.83 & \multicolumn{2}{c|}{x23.26} \\ \cline{6-11} 
\multirow{-5}{*}{OPQ'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Codebook\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{3.25W32A} & 76.41 & \multicolumn{2}{c|}{x38.03} \\ \hline

\end{tabular}
}
\end{table}

==> Table_new.tex <==


\begin{table}[hbt!]
\caption{Some results of RL-based and gradient-based (underlined) mixed precision frameworks, where at least weights have mixed precision.}
\label{tab:my-table11}
\resizebox{\textwidth}{!}
{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Framework & \begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular} & \begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular} & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Top 1\%\\ Accuracy\end{tabular} & Savings \\ \hline
\multirow{3}{*}{ReLeQ*} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{3}{*}{None} & ImageNet & AlexNet & 63.22 & 3.95x (speedup) \tablefootnote{\label{fn1}On conventional hardware using TVM compiler. Baseline: 8-bit precision models for inference} \\ \cline{4-7} 
 &  &  & Cifar-10 & VGG-16 & 93.46 & - \\ \cline{4-7} 
 &  &  & MNIST & LeNet & 99.4 & 2.76x (speedup) \footref{fn1}\\ \hline
\multirow{3}{*}{HAQ} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{3}{*}{Mixed} & \multirow{3}{*}{ImageNet} & ResNet-50 & 76.14 \tablefootnote{With model size constraints} & 8.03x (Model Size) \tablefootnote{\label{fn2}Baseline: 8W8A models with energy and latency constraints, 32W32A models with model size constraint} \\ \cline{5-7} 
 &  &  &  & MobileNet-V1 \tablefootnote{BitFusion} & 70.90 \tablefootnote{With energy constraints} & 1.16x (Energy) \footref{fn2} \\ \cline{5-7} 
 &  &  &  & MobileNet-V2 \tablefootnote{BISMO Edge accelerator} & 71.89 \tablefootnote{With latency constraints} & 1.4x (Latency) \footref{fn2} \\ \hline
AutoQ & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \end{tabular} & Mixed & ImageNet & ResNet-50 & 74.47 \tablefootnote{With resource-constraints} & 3.86x (Latency) \tablefootnote{Baseline: 16W16F models} \\ \hline
ADRL* & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \end{tabular} & {None} & ImageNet & ResNet-50 & 83.2 & 10x (Model Size) \tablefootnote{\label{bl}Baseline: 32W32F} \\ \hline
\multirow{2}{*}{\underline{SLWP}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & AlexNet \tablefootnote{1st layer is kept in full precision} & 52.54 \tablefootnote{Precision budget: 56} & - \\ \cline{4-7} 
 &  &  & MNIST & Similar to LeNet-5 & 98.86 \tablefootnote{Precision budget: 40} & - \\ \hline
\multirow{2}{*}{\underline{DQ}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet \tablefootnote{\label{memconst}Without constraints, and the networks are initialized with a pre-trained floating point network} & ResNet-18 \tablefootnote{\label{uniform}With best parametrization of uniform DQ} & 70.66 & 4.24x (Model Size)\tablefootnote{In terms of weight compression. Baseline: 32W32A models\label{w-s}}\\ \cline{4-7} 
 &  &  & Cifar-10 \footref{memconst} & ResNet-20 \footref{uniform} & 92.60 & - \\ \hline
\underline{OBACWA} & \begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular} & Mixed & ImageNet & ResNet-50 & 74.8 & 4x (Model Size) \footref{bl} \\ \hline
\multirow{3}{*}{\underline{Bayesian Bits}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{3}{*}{Mixed} & ImageNet & MobileNet-V2 & 72.00 \tablefootnote{\label{logit}Output logits left in full precision} & 16x (GbOp) \footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & VGG-7 & 93.23 \footref{logit} & 196.08x (GbOp) \footref{bl} \\ \cline{4-7} 
 &  &  & MNIST & LeNet-5 & 99.30 \footref{logit} & 277.78x (GbOp)\footref{bl} \\ \hline
 \end{tabular}
}
\end{table}



\begin{table}[hbt!]
\caption{Some results of heuristic-based mixed precision frameworks, where at least weights have mixed precision.}
\label{tab:my-table12}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Framework & \begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular} & \begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular} & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Top 1\%\\ Accuracy\end{tabular} & Savings \\ \hline
AQ & \begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular} & None & ImageNet & ResNet-50 \tablefootnote{Fully connected layers are kept in 16-bit precision} & 99.71 & 1.18x (Model Size)\tablefootnote{Baseline: Equal bit-width quantized model across all layers} \\ \hline
\multirow{3}{*}{PDB} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\end{tabular}} & \multirow{3}{*}{Fixed} & ImageNet & ResNet-18 \tablefootnote{The weights of
the input and output layers are left in full precision} & 65.03 & - \\ \cline{4-7} 
 &  &  & Cifar-10 & VGG-7 \tablefootnote{\label{pdb}The weights of the output layer are left in full precision} & 93.22 \tablefootnote{\label{manual}With manual fine-tuning} & - \\ \cline{4-7} 
 &  &  & Cifar-100 & VGG-7 \footref{pdb} & 71.53 \footref{manual} & - \\ \hline
HAWQ-V2 & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & Inception-V3 & 75.98 & 12.04x (Model Size)\footref{w-s} \\ \hline
\multirow{3}{*}{HAWQ-V3} &\multirow{3}{*}{ \begin{tabular}[c]{@{}c@{}}Retraining/\\Post-training\\ Deterministic\end{tabular}} & \multirow{3}{*}{Fixed/Mixed} & \multirow{3}{*}{ImageNet} & \multirow{3}{*}{ResNet-50} \tablefootnote{All results reported with distillation} & 77.58 & 1.15x (Model Size)\tablefootnote{Baseline: INT8 for weights and activations, with high model size constraint} \\ 
\cline{6-7} 
 &  &  &  &  & 76.97 & 1.13x (Speed)\tablefootnote{Baseline: INT8 for weights and activations, with high latency constraint} \\ 
\cline{6-7} 
 &  &  &  &  & 76.76 & 1.25x (BOPS)\tablefootnote{Baseline: INT8 for weights and activations, with high BOPS constraint} \\
\hline
\multirow{2}{*}{Hybrid-Net*} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic
\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & ResNet-18 & 62.73 & 0.20x (Memory Compression)\tablefootnote{\label{mc1}Baseline: XNOR network}\\ \cline{4-7} 
 &  &  & Cifar-100 & \begin{tabular}[c]{@{}c@{}}ResNet-32 \tablefootnote{\label{identity}With identity shortcut connections at each layer}\\ \tablefootnote{\label{res2}1st and last layer are kept in full precision}\end{tabular} & 64.45 & 0.31x (Memory Compression)\footref{mc1}\\ \hline
\multirow{2}{*}{ZeroQ} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular}} & \multirow{2}{*}{Fixed} & ImageNet & Inception-V3 & 78.76 & 5.34x (Model Size)\footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & ResNet-20 & 93.87 & \begin{tabular}[c]{@{}c@{}}5.20x\\ (Model Size)\\ \footref{bl}\end{tabular} \\ \hline
OPQ & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & None & ImageNet & ResNet-50 & 76.41 & 38.03x (Model Size)\footref{w-s} \\ \hline
MPQNNCO & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & ResNet-50 & 75.28 & 12.24x (Model Size)\footref{w-s} \\ \hline
\end{tabular}%
}
\end{table}



\begin{table}[h!]
\caption{Some results of meta-heuristic-based mixed precision frameworks, where at least weights have mixed precision.}
\label{tab:my-table13}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Framework & \begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular} & \begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular} & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Top 1\%\\ Accuracy\end{tabular} & Savings \\ \hline
\multirow{2}{*}{DNAS} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & \multirow{2}{*}{None/Mixed} & ImageNet & \begin{tabular}[c]{@{}c@{}}ResNet-34 \tablefootnote{\label{res3}ReLU-only preactivation}\\ \tablefootnote{\label{res1}Activations, the 1st and the last layer are kept in full precision}\end{tabular} & 74.61 & 10.6x (ModelSize)\footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & \begin{tabular}[c]{@{}c@{}}ResNet-110\\ \footref{res1}\end{tabular} & 95.07 & 12.5x (Model Size) \footref{bl} \\ \hline
\multirow{2}{*}{JASQ} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular}} & \multirow{2}{*}{None} & ImageNet & ResNet-152 \footref{res2} & 78.86 & 5.16x(Model Size) \footref{w-s} \\ \cline{4-7} 
 &  &  & Cifar-10 & JASQNet & 97.1 & - \\ \hline
\multirow{2}{*}{MPNASEE} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & Theirs-Base & 71.77 & \begin{tabular}[c]{@{}c@{}}2.67x (Energy)\\ 2.99x (Latency) \tablefootnote{\label{mbnet}Baseline: 8-bit precision quantized MobileNet-V2}\end{tabular} \\ \cline{4-7} 
 &  &  & Cifar-100 & Theirs-Base & 78.73 & \begin{tabular}[c]{@{}c@{}}4.21x (Energy)\\ 4.41x (Latency) \footref{mbnet}\end{tabular} \\ \hline
APQ & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & Their model  & 75.1 & 1.23x (BitOp)\footref{mbnet}\\ \hline
\multirow{2}{*}{BP-NAS} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retraining \\ Deterministic\end{tabular}} & \multirow{2}{*}{Mixed} & ImageNet & ResNet-50 & 76.67 & 71.65x (BitOp)\footref{bl} \\ \cline{4-7} 
 &  &  & Cifar-10 & ResNet-20 & 92.30 & 10.19x (Model Size)\footref{w-s}\\ \hline
{HMQ} & {\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular}} & {Mixed} & ImageNet & ResNet-50 & 75.73 & 11.1x (Model Size)\footref{w-s} \\ \hline
 %&  &  & Cifar-10 & ResNet-18 & 92.43 & \begin{tabular}[c]{@{}c@{}}11.06x\\ (Model\\Size)\footref{w-s}\end{tabular} \\ \hline
EdMIPS & \begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\end{tabular} & Mixed & ImageNet & Inception-V3 & 72.4 & 3.85x (Model Size)\tablefootnote{Using efficient composite convolution with respect to vanilla parallel convolutions} \\ \hline
EvoQ & \begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\end{tabular} & Fixed & ImageNet & ResNet-101 & 76.76 & 8x (Model Size) \footref{w-s}\\ \hline
Bit-Mixer & \begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\end{tabular} & Mixed & ImageNet & ResNet-50 \tablefootnote{Random per layer bit width selection} & 73.2 & - \\ \hline
\end{tabular}%
}
\end{table}

==> Table_old.tex <==
\begin{table}[]
\centering
\caption{Summary of Mixed Precision Frameworks, where at least weights are quantized with mixed bit precision. In "XWYA", "XW" and "YA" stand for the (average) \# of bits of weights and activations respectively. "X"/"Y"="F" when "W"/"A" take "Flexible" precision assignments layer-wise. "QOP"=quantization as an optimization problem. "DS"=Differentiable Search. "ES"=Evolutionary Search.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\ Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Precision Budget\\ (in bits)\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 97.68 & \multicolumn{2}{c|}{10} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 98.31 & \multicolumn{2}{c|}{20} \\ \cline{7-11} 
 &  &  &  & \multirow{-3}{*}{MNIST} & \multirow{-3}{*}{Similar to LeNet-5} & \multicolumn{2}{c|}{8W8A} & 98.86 & \multicolumn{2}{c|}{40} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{2W2A} & 51.46 & \multicolumn{2}{c|}{14} \\ \cline{7-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 52.31 & \multicolumn{2}{c|}{28} \\ \cline{7-11} 
\multirow{-7}{*}{SLWP'18} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-7}{*}{Mixed} & \multirow{-3}{*}{ImageNet} & \multirow{-3}{*}{AlexNet \footnote{1st layer is kept in full precision}} & \multicolumn{2}{c|}{8W8A} & 52.54 & \multicolumn{2}{c|}{56} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\% \\Accuracy \end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\Savings \footnote{Baseline: Equal bit-width quantized models across all layers}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet \footnote{\label{fc16}Fully connected layers are kept in 16-bit precision} & \multicolumn{2}{c|}{FW32A} & 99.50 & \multicolumn{2}{c|}{x1.84} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.68 & \multicolumn{2}{c|}{x1.68} \\ \cline{6-11} 
 &  &  &  &  & GoogLeNet \footref{fc16} & \multicolumn{2}{c|}{FW32A} & 99.60 & \multicolumn{2}{c|}{x1.16} \\ \cline{6-11} 
\multirow{-5}{*}{AQ'18} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 \footref{fc16}& \multicolumn{2}{c|}{FW32A} & 99.71 & \multicolumn{2}{c|}{x1.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ (or Computational) \footnote{When activations are quantized along with the weights, the computational savings are reported rather than model size savings}\\ Savings \footnote{\label{size}Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{} & 92.72 & \multicolumn{2}{c|}{x16.6} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-56 & \multicolumn{2}{c|}{} & 94.57 & \multicolumn{2}{c|}{x18.93} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-3}{*}{Cifar-10} & ResNet-110 & \multicolumn{2}{c|}{\multirow{-3}{*}{FW32A \footnote{\label{res1}Activations, the 1st and the last layer are kept in full precision}}} & 95.07 & \multicolumn{2}{c|}{x20.3} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 71.21 & \multicolumn{2}{c|}{x21.1} \\ \cline{7-11} 
 &  &  &  &  & \multirow{-2}{*}{ResNet-18 \footnote{\label{res3}ReLU-only preactivation}} & \multicolumn{2}{c|}{FWFA \footnote{\label{res2}1st and last layer are kept in full precision}} & 71.01 & \multicolumn{2}{c|}{x103.5} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{FW32A \footref{res1}} & 74.61 & \multicolumn{2}{c|}{x19.0} \\ \cline{7-11} 
\multirow{-8}{*}{DNAS'18} & \multirow{-8}{*}{DS} & \multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-8}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \multirow{-2}{*}{ResNet-34 \footref{res3}} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 74.21 & \multicolumn{2}{c|}{x87.4} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footnote{\label{accloss}Compared to the full precision model}\end{tabular} & \multicolumn{2}{c|}{Speedup \footnote{On conventional hardware using TVM compiler. Baseline: 8-bit precision models for inference}} \\ \cline{5-11} 
 &  &  &  & ImageNet & AlexNet & \multicolumn{2}{c|}{5W32A} & 0.08 & \multicolumn{2}{c|}{x3.95} \\ \cline{5-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{6.43W32A} & 0.26 & \multicolumn{2}{c|}{x1.24} \\ \cline{5-11} 
 &  &  &  &  & SimpleNet & \multicolumn{2}{c|}{5W32A} & 0.30 & \multicolumn{2}{c|}{x1.92} \\ \cline{6-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{2.81W32A} & 0.12 & \multicolumn{2}{c|}{x3.27} \\ \cline{6-11} 
 &  &  &  &  & VGG-11 & \multicolumn{2}{c|}{6.44W32A} & 0.17 & \multicolumn{2}{c|}{x1.53} \\ \cline{6-11} 
 &  &  &  & \multirow{-4}{*}{Cifar-10} & VGG-16 & \multicolumn{2}{c|}{7.25W32A} & 0.10 & \multicolumn{2}{c|}{-} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet & \multicolumn{2}{c|}{2.25W32A} & 0.00 & \multicolumn{2}{c|}{x2.76} \\ \cline{5-11} 
\multirow{-9}{*}{ReLeQ'18} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}LSTM-based\\ RL\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{None} & SVHN & SVHN-10 & \multicolumn{2}{c|}{4.8W32A} & 100 & \multicolumn{2}{c|}{x2.18} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{The weights of the output layer are left in full precision in experiments on CIFAR-10\/100 and Pascal VOC, and the weights of the input and output layers are left in full precision in the experiments on ImageNet}\end{tabular}} & \multicolumn{3}{c|}{Top-1\% Accuracy} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{W4A} & \multicolumn{3}{c|}{90.54} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-10} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{93.22} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{3.82W4A} & \multicolumn{3}{c|}{64.28} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{CIFAR-100} & VGG-7 & \multicolumn{2}{c|}{1.06W2A} & \multicolumn{3}{c|}{71.53} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{1.10W2A} & \multicolumn{3}{c|}{53.18} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{1.42W2A} & \multicolumn{3}{c|}{65.03} \\ \cline{5-11} 
 &  &  &  &  & SSD-300 & \multicolumn{2}{c|}{1.22W2A} & \multicolumn{3}{c|}{62.21} \\ \cline{6-11} 
\multirow{-9}{*}{PDB'19} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based on\\ input separability\end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-9}{*}{Fixed} & \multirow{-2}{*}{Pascal VOC} & Faster R-CNN & \multicolumn{2}{c|}{1.52W4A} & \multicolumn{3}{c|}{74.52} \\ \hline
{\color[HTML]{000000} } &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
{\color[HTML]{000000} } &  &  &  & Cifar-10 \footnote{\label{memconst}Without constraints, and the networks are initialized with a pre-trained floating point network} & ResNet-20 \footnote{\label{uniform}With best parametrization of uniform DQ} & \multicolumn{2}{c|}{} & 92.60 & \multicolumn{2}{c|}{-} \\ \cline{5-6} \cline{9-11} 
{\color[HTML]{000000} } &  &  &  &  & MobileNet-V2 \footref{uniform} & \multicolumn{2}{c|}{} & 70.59 & \multicolumn{2}{c|}{x4.21} \\ \cline{6-6} \cline{9-11} 
\multirow{-4}{*}{{\color[HTML]{000000} DQ'19}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & \multirow{-2}{*}{ImageNet \footref{memconst}} & ResNet-18 \footref{uniform} & \multicolumn{2}{c|}{\multirow{-3}{*}{FWFW}} & 70.66 & \multicolumn{2}{c|}{x4.24} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Constraint\end{tabular} & \begin{tabular}[c]{@{}c@{}}Budget\\ Savings \footnote{Baseline: 8W8A models with energy and latency constraints, 32W32A models with model size constraint}\end{tabular} \\ \cline{5-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{edge}Edge Accelerator} & \multicolumn{2}{c|}{6.8W5.42A} & 70.58 &  & x1.66 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{cloud}Cloud Accelerator} & \multicolumn{2}{c|}{5.73W4.77A} & 69.97 &  & x1.95 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V1 \footnote{\label{bitfusion}BitFusion} & \multicolumn{2}{c|}{FWFA} & 70.40 &  & x1.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{edge} & \multicolumn{2}{c|}{5.86W6.10A} & 71.89 &  & x1.4 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 \footref{cloud} & \multicolumn{2}{c|}{4.92W5.29A} & 71.85 & \multirow{-5}{*}{Latency} & x1.45 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 \footref{bitfusion} & \multicolumn{2}{c|}{FWFA} & 70.37 & Energy & x1.9 \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FWFA} & 71.74 &  & x7.8 \\ \cline{6-9} \cline{11-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{3.85WFA} & 71.47 &  & x7.47 \\ \cline{6-9} \cline{11-11} 
\multirow{-10}{*}{HAQ'19} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}RL w/\\ budget constraints\end{tabular}} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding/\\ Vector Quant.\end{tabular}} & \multirow{-10}{*}{Mixed} & \multirow{-9}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 76.14 & \multirow{-3}{*}{Model Size} & x8.03 \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{w-s}In terms of weight compression. Baseline: 32W32A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & Cifar-10 & ResNet-20 & \multicolumn{2}{c|}{4.05W4A \footnote{fixed 4 bits are used for activations in all layers except the 1st and last, where 8 bits are used}} & 92.22 & \multicolumn{2}{c|}{x13.11} \\ \cline{5-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{3.43W4.11A} & 75.52 & \multicolumn{2}{c|}{x12.04} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.48 & \multicolumn{2}{c|}{x12.28} \\ \cline{6-11} 
\multirow{-5}{*}{HAWQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hessian\\ Spectrum\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Fixed/Mixed} & \multirow{-3}{*}{ImageNet} & SqueezeNet & \multicolumn{2}{c|}{FWFA} & 68.02 & \multicolumn{2}{c|}{x9.25} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits \footnote{\label{kernel}Kernel-wise quantization results are reported}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footnote{Baseline: 16W16F models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{3.32W4.12A} & 30.22 & \multicolumn{2}{c|}{x4.06} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4.02W3.93A} & 25.53 & \multicolumn{2}{c|}{x3.86} \\ \cline{6-11} 
 &  &  &  &  & SqueezeNet-V1 & \multicolumn{2}{c|}{3.76W4.05A} & 43.51 & \multicolumn{2}{c|}{x3.06} \\ \cline{6-11} 
\multirow{-5}{*}{AutoQ'19} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Hierarchical\\ deep RL\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{3.67W4.14A} & 29.21 & \multicolumn{2}{c|}{xx3.42} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 \footnote{\label{1stlast}1st and last layer are kept in full precision} & \multicolumn{2}{c|}{FW32A} & 69.60 & \multicolumn{2}{c|}{x13.9} \\ \cline{6-11} 
 &  &  &  & \multirow{-2}{*}{ImageNet} & MobileNet-V2 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 71.65 & \multicolumn{2}{c|}{x9.1} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 92.27 & \multicolumn{2}{c|}{x28.3} \\ \cline{6-11} 
 &  &  &  &  & ResNet-56 \footref{1stlast} \footnote{With cutout operation} & \multicolumn{2}{c|}{FW32A} & 94.48 & \multicolumn{2}{c|}{x23.2} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-10} & MobileNet-V2 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 93.28 & \multicolumn{2}{c|}{x12.4} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 68.18 & \multicolumn{2}{c|}{x11.6} \\ \cline{6-11} 
 &  &  &  &  & Res-Net-56 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 71.84 & \multicolumn{2}{c|}{x17.2} \\ \cline{6-11} 
\multirow{-9}{*}{CBAQ'19} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Cursor-based\\ DS \end{tabular}} & \multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-9}{*}{None} & \multirow{-3}{*}{CIFAR-100} & MobileNet-V2 \footref{1stlast} & \multicolumn{2}{c|}{FW32A} & 68.04 & \multicolumn{2}{c|}{x12.9} \\ \hline
 \end{tabular}%
}
%\afterpage{\clearpage}
\end{table}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|l|c|c|c|}
\hline
 &  &  &  & \multicolumn{7}{c|}{Benchmarks} \\ \cline{5-11} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Precision\\ Framework\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Optimization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Quantization\\Technique\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Activation\\ Quantization\end{tabular}} & Dataset(s) & Model(s) & \multicolumn{5}{c|}{Metrics} \\
\hline
  &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ Savings \footnote{\label{mbnet}Baseline: 8-bit precision quantized MobileNet-V2}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Latency\\ Savings \footref{mbnet}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-100 & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 68.38 & x3.26 & x3.49 \\ \cline{5-11} 
\multirow{-3}{*}{MPNASEE'19} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ \\ energy constraints\\ and a proxy task\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Theirs-Small & \multicolumn{2}{c|}{FWFA} & 77.84 & x5.09 & x5.19 \\ \hline
&  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Giga Bit\\ Operation \\ Count Savings \footnote{Of full precision model}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet-5 & \multicolumn{2}{c|}{FWFA} & 99.30 & \multicolumn{2}{c|}{x277.78} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & VGG-7 & \multicolumn{2}{c|}{FWFA} & 93.23 & \multicolumn{2}{c|}{x196.08} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 69.36 & \multicolumn{2}{c|}{x51.81} \\ \cline{6-11} 
\multirow{-5}{*}{Bayesian Bits'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Variational\\ inference\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{FWFA} & 72 & \multicolumn{2}{c|}{x16} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top 1-\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Bit Operations\\ Savings \footnote{Baseline: 4W4A models}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 \footnote{\label{res-blocks}Only res-blocks are searched and quantized; excluding the 1st convolution layer and last fully connected layer} & \multicolumn{2}{c|}{FWFA} & 70.50 & \multicolumn{2}{c|}{x1.04} \\ \cline{6-11} 
\multirow{-3}{*}{SPOSNAS'20} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}ES w/ budget\\ constraints\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & ResNet-34 \footref{res-blocks} & \multicolumn{2}{c|}{FWFA} & 74.60 & \multicolumn{2}{c|}{x1.02} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top 1-\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Bit Operations\\ Savings \footref{mbnet}\end{tabular}} \\ \cline{5-11} 
\multirow{-3}{*}{APQ'20} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Predictor-based\\ES w/ budget\\ constraints\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-3}{*}{Mixed} & ImageNet & Their joint designed models & \multicolumn{2}{c|}{FWFA} & 75.1 & \multicolumn{2}{c|}{x1.23} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy (or mAP) \footnote{mAP is used for COCO dataset}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bit Operations\\ Budget\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{4W3.9A} & 92.30 & 4 & x10.19 \\ \cline{5-11} 
 &  &  &  & ImageNet & ResNet-50 & \multicolumn{2}{c|}{-} & 76.67 & 4 & - \\ \cline{5-11} 
\multirow{-4}{*}{BP-NAS'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}DS w/ complexity\\ constraints\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining \\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Mixed} & Microsoft COCO & \begin{tabular}[c]{@{}c@{}}ResNet-50 \\ (faster R-CNN)\end{tabular} & \multicolumn{2}{c|}{3.84W4.31A} & 0.358 & 4 & - \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Memory\\ Savings \footnote{Baseline: XNOR network}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 \footnote{\label{identity}With identity shortcut connections at each layer} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.88 & \multicolumn{2}{c|}{0.53} \\ \cline{6-11} 
 &  &  &  &  & ResNet-32 \footref{identity} & \multicolumn{2}{c|}{FWFA \footref{res2}} & 64.45 & \multicolumn{2}{c|}{0.69} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-100} & VGG-15 & \multicolumn{2}{c|}{FWFA \footref{res2}} & 63.38 & \multicolumn{2}{c|}{0.50} \\ \cline{5-11} 
\multirow{-5}{*}{Hybrid-Net'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Heuristic based\\ on PCA\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & ImageNet & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 62.73 & \multicolumn{2}{c|}{0.80} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 92.43 & \multicolumn{2}{c|}{x11.06} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FWFA} & 75.45 & \multicolumn{2}{c|}{x13.1} \\ \cline{6-11} 
 &  &  &  &  & EfficientNet-B0 & \multicolumn{2}{c|}{FW8A} & 74.6 & \multicolumn{2}{c|}{x11.97} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{FW8A} & 69.88 & \multicolumn{2}{c|}{x10.68} \\ \cline{6-11} 
\multirow{-6}{*}{HMQ'20} & \multirow{-6}{*}{DS} & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic \\ Rounding\end{tabular}} & \multirow{-6}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & MobileNet-V2 & \multicolumn{2}{c|}{FWFA} & 70.9 & \multicolumn{2}{c|}{x8.05} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{Using efficient composite convolution with respect to vanilla parallel convolutions}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{AlexNet} & \multicolumn{2}{c|}{2W2A} & 59.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{-}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & 68 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & 67 & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-18} & \multicolumn{2}{c|}{2W2A} & 65.9 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{GoogLeNet} & \multicolumn{2}{c|}{2W2A} & 67.8 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.45}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  & \multirow{-3}{*}{ResNet-50} & \multicolumn{2}{c|}{2W2A} & 72.1 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \cline{6-11} 
 &  &  &  &  &  & \multicolumn{2}{c|}{4W4A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
 &  &  &  &  &  & \multicolumn{2}{c|}{3W3A} & - & \multicolumn{2}{c|}{} \\ \cline{7-9}
\multirow{-16}{*}{EdMIPS'20} & \multirow{-16}{*}{DS} & \multirow{-16}{*}{\begin{tabular}[c]{@{}c@{}}Training-aware\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-16}{*}{Mixed} & \multirow{-15}{*}{ImageNet} & \multirow{-3}{*}{Inception-V3} & \multicolumn{2}{c|}{2W2A} & 72.4 & \multicolumn{2}{c|}{\multirow{-3}{*}{x3.85}} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{size}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{} & 77.43 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & MobileNet-V2 & \multicolumn{2}{c|}{} & 72.85 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ShuffleNet & \multicolumn{2}{c|}{} & 62.90 & \multicolumn{2}{c|}{x5.35} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & ResNet-152 & \multicolumn{2}{c|}{} & 77.88 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & Inception-V3 & \multicolumn{2}{c|}{} & 78.76 & \multicolumn{2}{c|}{x5.34} \\ \cline{6-6} \cline{9-11} 
 &  &  &  &  & SqueezeNext & \multicolumn{2}{c|}{} & 68.17 & \multicolumn{2}{c|}{x5.33} \\ \cline{6-6} \cline{9-11} 
 &  &  &  & \multirow{-7}{*}{ImageNet} & ResNet-18 & \multicolumn{2}{c|}{} & 71.30 & \multicolumn{2}{c|}{x5.34} \\ \cline{5-6} \cline{9-11} 
 &  &  &  & Cifar-10 & ResNet-20 & \multicolumn{2}{c|}{} & 93.87 & \multicolumn{2}{c|}{x5.20} \\ \cline{5-6} \cline{9-11} 
\multirow{-10}{*}{ZeroQ'20} & \multirow{-10}{*}{Pareto Frontier} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Post-training\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-10}{*}{Fixed} & Microsoft COCO & RetinaNet & \multicolumn{2}{c|}{\multirow{-9}{*}{FW6A}} & 35.9 & \multicolumn{2}{c|}{x6.00} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy \footnote{Reported for EBS with deterministic search}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Computational\\ Savings \footnote{In terms of FLOPs}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-20 & \multicolumn{2}{c|}{FWFA} & 92.94 & \multicolumn{2}{c|}{x4.01} \\ \cline{6-11} 
 &  &  &  &  & ResNet-32 & \multicolumn{2}{c|}{FWFA} & 93.53 & \multicolumn{2}{c|}{x3.24} \\ \cline{6-11} 
 &  &  &  & \multirow{-3}{*}{CIFAR-10} & ResNet-56 & \multicolumn{2}{c|}{FWFA} & 94.27 & \multicolumn{2}{c|}{x3.76} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & 70.20 & \multicolumn{2}{c|}{x3.26} \\ \cline{6-11} 
\multirow{-6}{*}{EBS'20} & \multirow{-6}{*}{DS} & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-6}{*}{Mixed} & \multirow{-2}{*}{ImageNet} & ResNet-34 & \multicolumn{2}{c|}{FWFA} & 73.50 & \multicolumn{2}{c|}{x3.33} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & MNIST & LeNet5 \footnote{Based on \cite{}} & \multicolumn{2}{c|}{-} & 99.12 & \multicolumn{2}{c|}{x75.77} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & VGG \footnote{Based on \cite{}} & \multicolumn{2}{c|}{0.66W32A} & 92.00 & \multicolumn{2}{c|}{x43.48} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{2W32A} & 68.90 & \multicolumn{2}{c|}{x13.58} \\ \cline{6-11} 
\multirow{-5}{*}{ALQ'20} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Vector Quant.\end{tabular}} & \multirow{-5}{*}{Fixed/None} & \multirow{-2}{*}{ImageNet} & ResNet-34 & \multicolumn{2}{c|}{2W2A} & 71.00 & \multicolumn{2}{c|}{x13.68} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}\% Accuracy\\ Loss \footref{accloss}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footnote{\label{bl}Baseline: 32W32F}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.30} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.10} \\ \cline{6-11} 
\multirow{-4}{*}{ADRL'20} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Deep RL w/\\ compression\\ ratio constraint\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{None} & \multirow{-2}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{FW32A} & 0 & \multicolumn{2}{c|}{x10.00} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \multicolumn{3}{c|}{Top-1\% Accuracy \footnote{Random per layer bit selection}} \\ \cline{5-11} 
 &  &  &  &  & ResNet-18 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{65.8} \\ \cline{6-11} 
 &  &  &  &  & ResNet-34 & \multicolumn{2}{c|}{FWFA} & \multicolumn{3}{c|}{70.5} \\ \cline{6-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{73.2} \\ \cline{6-11} 
\multirow{-5}{*}{Bit-Mixer'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}3-stage\\ optimization on\\ Meta-Network\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-5}{*}{Mixed} & \multirow{-4}{*}{ImageNet} & \begin{tabular}[c]{@{}c@{}}EBN \\ 4:4:4:4\end{tabular} & \multicolumn{2}{c|}{4W4A} & \multicolumn{3}{c|}{72.1} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Average \#\\ of Bits\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{w-s}\end{tabular}} \\ \cline{5-11} 
 &  &  &  &  & AlexNet & \multicolumn{2}{c|}{2.99W32A} & 57.09 & \multicolumn{2}{c|}{x138.96} \\ \cline{6-11} 
 &  &  &  &  & VGG-16 & \multicolumn{2}{c|}{2.92W32A} & 71.39 & \multicolumn{2}{c|}{x195.87} \\ \cline{6-11} 
 &  &  &  &  & MobileNet-V1 & \multicolumn{2}{c|}{3.26W32A} & 70.83 & \multicolumn{2}{c|}{x23.26} \\ \cline{6-11} 
\multirow{-5}{*}{OPQ'21} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Codebook\end{tabular}} & \multirow{-5}{*}{None} & \multirow{-4}{*}{ImageNet} & ResNet-50 & \multicolumn{2}{c|}{3.25W32A} & 76.41 & \multicolumn{2}{c|}{x38.03} \\ \hline
 &  &  &  & \notableentry & \notableentry & \multicolumn{2}{c|}{\# of Bits} & \begin{tabular}[c]{@{}c@{}}Top-1\%\\ Accuracy\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ Savings \footref{bl}\end{tabular}} \\ \cline{5-11} 
 &  &  &  & CIFAR-10 & ResNet-20 & \multicolumn{2}{c|}{FW4A \footnote{\label{activate}First and last layer activations are left as 8-bit precision}} & 92.32 & \multicolumn{2}{c|}{x14.24} \\ \cline{5-11} 
 &  &  &  &  & ResNet-50 & \multicolumn{2}{c|}{FW4A \footref{activate}} & 75.29 & \multicolumn{2}{c|}{x11.90} \\ \cline{6-11} 
\multirow{-4}{*}{BSQ'21} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Constrained\\ Heuristic\end{tabular}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Retraining\\ Deterministic\\ Rounding\end{tabular}} & \multirow{-4}{*}{Fixed} & \multirow{-2}{*}{ImageNet} & Inception-V3 & \multicolumn{2}{c|}{FW6A} & 76.60 & \multicolumn{2}{c|}{x11.38} \\ \hline
\end{tabular}
}
\end{table}

==> test.tex <==
\begin{landscape}
\begin{figure}
\vspace{-1cm}
\centering
\begin{tikzpicture}
\path[mindmap,concept color=black,text=white]
    node[concept] {Mixed Precision\\ Frameworks}
    [clockwise from=140]
    
    child[concept color=orange, yshift=-3.5cm, grow=-180,font=\fontsize{10pt}{16pt}]{ 
        node[concept] {Gradient-Based\\Optimization}
            [clockwise from=-60]
        % child {node[concept] {\cite{}} }
        child {node[concept] {SLWP(\cite{lacey2018stochastic})} }
        child {node[concept] {DQ (\cite{uhlich2019differentiable})} }
        child {node[concept] {Bayesian Bits (\cite{van2020bayesian})}
        }}
    child[concept  color=orange, grow=-90, xshift=2cm,] 
    { 
        node[concept] {Heuristic-Based\\Optimization}
            [clockwise from=-40]
        % child {node[concept] {\cite{}} }
        child {node[concept] {AQ(\cite{zhou2018adaptive})} }
        child {node[concept] {PDB (\cite{chu2019mixed})} }
        child {node[concept] {HAWQ (\cite{dong2019hawq})}}
        child {node[concept] {Hybrid-Net (\cite{chakraborty2020constructing})}}  
        child {node[concept] {ZeroQ (\cite{cai2020zeroq})}}
        child {node[concept] {OPQ (\cite{hu2021opq})}
        } }
    child[concept  color=orange, grow=10, xshift=2cm,font=\fontsize{10pt}{16pt}]
    { 
        node[concept] {Meta-Heuristic-Based\\Optimization}
            [clockwise from=-90]
        child {node[concept]{DNAS (\cite{wu2018mixed})} }
        child {node[concept] {MPNASEE (\cite{pan2019})} }
        child {node[concept] {APQ (\cite{wang2020apq})}}
        child {node[concept] {BP-NAS (\cite{yu2020search})}}
        child {node[concept] {HMQ (\cite{habi2020hmq})}}
        child {node[concept] {EdMIPS (\cite{cai2020rethinking})}}
        child {node[concept] {Bit-Mixer (\cite{bulat2021bit})}}
        };
\end{tikzpicture}
\label{mindmap}
\caption{Alternative approaches and different methods for approximating a CPE}
\end{figure}
\end{landscape}
 
 
\begin{comment}

\begin{tikzpicture}
\path[mindmap,concept color=black,text=white]
    node[concept] {Constant Phase\\ Element}
    [clockwise from=140]
    child[concept  color=orange, grow=-20, xshift=2cm,] { 
     node[concept  ,scale=1.5,font=\fontsize{10pt}{20pt}] {Emulators}
        child [concept color=black!40, grow=-170]{node[concept, scale=1.5,yshift=-2cm] {TF based Approx.}  
        [clockwise from=-110]
            child {node[concept,scale=1.5,yshift=-0.8cm] {Oustaloup\\ \cite{oustaloup1996crone} }}
            child {node[concept,scale=1.5,xshift=-0.6cm,yshift=-0.7cm] {Matsuda\\ \cite{khoichi1993h}} }
            child {node[concept,scale=1.5,xshift=-1cm,yshift=-0.4cm] {CFE\\ \cite{roy1967realization}}}
            child {node[concept,scale=1.5,xshift=-1cm,yshift=0.1cm] {Charef\\ \cite{charef1992fractal}} }
            child {node[concept,scale=1.5,xshift=-0.5cm,yshift=0.4cm] {Carlson\\ \cite{carlson1960simulation}} } }
        child [concept color=black!40, grow=-30] {node[concept,scale=1.5, xshift=1.5cm] {Circuit Inspired Approx.}
            child[concept color=red!60!black, grow=-90] {node[concept,scale=2, yshift=-1.5cm ] {Systematic \\ Synthesis}
            [clockwise from=60]
            child {node[concept,scale=2,xshift=0.5cm,yshift=0.5cm] {Valsa\\ \cite{valsa2011network} }}
            child {node[concept,scale=2,xshift=0.7cm,yshift=-0.2cm] {Morrison\\ \cite{morrison1959rc}} }
            child {node[concept,scale=2,xshift=0.3cm,yshift=-1.cm] {Sugi \\ \cite{sugi2002frequency}} } }
            child [concept color=yellow!60!black, grow=-135] {node[concept, scale=2, xshift=-1.2cm,yshift=-2.5cm] {Optimization} 
            [clockwise from=-30]
                child {node[concept,scale=2, xshift=0.7cm ] {Yousri\\ \cite{YOUSRI2019110}} }
                child {node[concept,scale=2, xshift=0, yshift=-0.7cm ] {Oshakov\\ \cite{ARKHIPOVICHUSHAKOV2020}} }
                child {node[concept,scale=2, xshift=-0.7cm, yshift=-0.7cm ] {Kartci \cite{kartci2019synthesis}} }
                child [concept color=green!60!blue] {node[concept,scale=2, xshift=-1cm, yshift=0cm ] {This \\ Work} }
            }
    }}
    child[concept color=orange, yshift=-3.5cm, grow=180,font=\fontsize{10pt}{16pt}]{ 
        node[concept] {Fabrication}
            [clockwise from=-60]
        % child {node[concept] {\cite{}} }
        child {node[concept] {Fractal structure  \cite{jesus2009development,598289,haba2005influence}} }
        child {node[concept] {polymers \cite{caponetto2013experimental,agambayev2018ultra}} }
        child {node[concept] {Solid-state \cite{BUSCARINO2018307,john2017solid,adhikary2015realization,elshurafa2013microscale}} }
        child {node[concept] {Electro-chemical \cite{1705043,6262466}} }
    };
\end{tikzpicture}
\label{mindmap}
\caption{Alternative approaches and different methods for approximating a CPE}

\end{comment}
